Measurement of the $\eta_c(1S)$ production cross-section in $pp$ collisions at $\sqrt{s} = 13$ TeV

Using a data sample corresponding to an integrated luminosity of $2.0\,fb^{-1}$, collected by the LHCb experiment, the production of the $\eta_c(1S)$ state in proton-proton collisions at a centre-of-mass energy of $\sqrt{s}=13 \text{ TeV}$ is studied in the rapidity range ${2.0 < y < 4.5}$ and in the transverse momentum range ${6.5 < p_{T} < 14.0\text{ GeV}}$. The cross-section for prompt production of $\eta_c(1S)$ mesons relative to that of the $J/\psi$ meson is measured using the ${p\bar{p}}$ decay mode and is found to be ${\sigma_{\eta_c(1S)}/\sigma_{J/\psi} = 1.69 \pm 0.15 \pm 0.10 \pm 0.18}$. The quoted uncertainties are, in order, statistical, systematic and due to uncertainties on the branching fractions of the ${J/\psi\to p \bar{p}}$ and ${\eta_c\to p \bar{p}}$ decays. The prompt $\eta_c(1S)$ production cross-section is determined to be ${\sigma_{\eta_c(1S)} = 1.26 \pm 0.11\pm 0.08 \pm 0.14 \,\mu b}$, where the last uncertainty includes that on the ${J/\psi}$ meson cross-section. The ratio of the branching fractions of $b$-hadron decays to the $\eta_c(1S)$ and ${J/\psi}$ states is measured to be ${\mathcal{B}_{b\to\eta_c X}/\mathcal{B}_{b\to J/\psi X} = 0.48 \pm 0.03 \pm 0.03 \pm 0.05}$, where the last uncertainty is due to those on the branching fractions of the ${J/\psi \to p \bar{p}}$ and ${\eta_c\to p \bar{p}}$ decays. The difference between the ${J/\psi}$ and $\eta_c(1S)$ masses is also determined to be ${113.0 \pm 0.7 \pm 0.1\text{ MeV}}$, which is the most precise single measurement of this quantity to date.

==> LHCb_Authorship_11-Jun-2019.tex <==
% LHCb collaboration author list
% Data extracted on June 11th, 2019 at 3:40pm for reference date 11-Jun-2019
\centerline
{\large\bf LHCb collaboration}
\begin
{flushleft}
\small
R.~Aaij$^{29}$,
C.~Abell{\'a}n~Beteta$^{46}$,
T.~Ackernley$^{56}$,
B.~Adeva$^{43}$,
M.~Adinolfi$^{50}$,
H.~Afsharnia$^{7}$,
C.A.~Aidala$^{78}$,
S.~Aiola$^{23}$,
Z.~Ajaltouni$^{7}$,
S.~Akar$^{61}$,
P.~Albicocco$^{20}$,
J.~Albrecht$^{12}$,
F.~Alessio$^{44}$,
M.~Alexander$^{55}$,
A.~Alfonso~Albero$^{42}$,
G.~Alkhazov$^{35}$,
P.~Alvarez~Cartelle$^{57}$,
A.A.~Alves~Jr$^{43}$,
S.~Amato$^{2}$,
Y.~Amhis$^{9}$,
L.~An$^{19}$,
L.~Anderlini$^{19}$,
G.~Andreassi$^{45}$,
M.~Andreotti$^{18}$,
F.~Archilli$^{14}$,
J.~Arnau~Romeu$^{8}$,
A.~Artamonov$^{41}$,
M.~Artuso$^{64}$,
K.~Arzymatov$^{39}$,
E.~Aslanides$^{8}$,
M.~Atzeni$^{46}$,
B.~Audurier$^{24}$,
S.~Bachmann$^{14}$,
J.J.~Back$^{52}$,
S.~Baker$^{57}$,
V.~Balagura$^{9,b}$,
W.~Baldini$^{18,44}$,
A.~Baranov$^{39}$,
R.J.~Barlow$^{58}$,
S.~Barsuk$^{9}$,
W.~Barter$^{57}$,
M.~Bartolini$^{21}$,
F.~Baryshnikov$^{74}$,
G.~Bassi$^{26}$,
V.~Batozskaya$^{33}$,
B.~Batsukh$^{64}$,
A.~Battig$^{12}$,
V.~Battista$^{45}$,
A.~Bay$^{45}$,
M.~Becker$^{12}$,
F.~Bedeschi$^{26}$,
I.~Bediaga$^{1}$,
A.~Beiter$^{64}$,
L.J.~Bel$^{29}$,
V.~Belavin$^{39}$,
S.~Belin$^{24}$,
N.~Beliy$^{4}$,
V.~Bellee$^{45}$,
K.~Belous$^{41}$,
I.~Belyaev$^{36}$,
G.~Bencivenni$^{20}$,
E.~Ben-Haim$^{10}$,
S.~Benson$^{29}$,
S.~Beranek$^{11}$,
A.~Berezhnoy$^{37}$,
R.~Bernet$^{46}$,
D.~Berninghoff$^{14}$,
E.~Bertholet$^{10}$,
A.~Bertolin$^{25}$,
C.~Betancourt$^{46}$,
F.~Betti$^{17,e}$,
M.O.~Bettler$^{51}$,
Ia.~Bezshyiko$^{46}$,
S.~Bhasin$^{50}$,
J.~Bhom$^{31}$,
M.S.~Bieker$^{12}$,
S.~Bifani$^{49}$,
P.~Billoir$^{10}$,
A.~Birnkraut$^{12}$,
A.~Bizzeti$^{19,u}$,
M.~Bj{\o}rn$^{59}$,
M.P.~Blago$^{44}$,
T.~Blake$^{52}$,
F.~Blanc$^{45}$,
S.~Blusk$^{64}$,
D.~Bobulska$^{55}$,
V.~Bocci$^{28}$,
O.~Boente~Garcia$^{43}$,
T.~Boettcher$^{60}$,
A.~Boldyrev$^{75}$,
A.~Bondar$^{40,y}$,
N.~Bondar$^{35}$,
S.~Borghi$^{58,44}$,
M.~Borisyak$^{39}$,
M.~Borsato$^{14}$,
J.T.~Borsuk$^{31}$,
M.~Boubdir$^{11}$,
T.J.V.~Bowcock$^{56}$,
C.~Bozzi$^{18,44}$,
S.~Braun$^{14}$,
A.~Brea~Rodriguez$^{43}$,
M.~Brodski$^{44}$,
J.~Brodzicka$^{31}$,
A.~Brossa~Gonzalo$^{52}$,
D.~Brundu$^{24,44}$,
E.~Buchanan$^{50}$,
A.~Buonaura$^{46}$,
C.~Burr$^{44}$,
A.~Bursche$^{24}$,
J.S.~Butter$^{29}$,
J.~Buytaert$^{44}$,
W.~Byczynski$^{44}$,
S.~Cadeddu$^{24}$,
H.~Cai$^{68}$,
R.~Calabrese$^{18,g}$,
S.~Cali$^{20}$,
R.~Calladine$^{49}$,
M.~Calvi$^{22,i}$,
M.~Calvo~Gomez$^{42,m}$,
A.~Camboni$^{42,m}$,
P.~Campana$^{20}$,
D.H.~Campora~Perez$^{44}$,
L.~Capriotti$^{17,e}$,
A.~Carbone$^{17,e}$,
G.~Carboni$^{27}$,
R.~Cardinale$^{21}$,
A.~Cardini$^{24}$,
P.~Carniti$^{22,i}$,
K.~Carvalho~Akiba$^{2}$,
A.~Casais~Vidal$^{43}$,
G.~Casse$^{56}$,
M.~Cattaneo$^{44}$,
G.~Cavallero$^{21}$,
R.~Cenci$^{26,p}$,
J.~Cerasoli$^{8}$,
M.G.~Chapman$^{50}$,
M.~Charles$^{10,44}$,
Ph.~Charpentier$^{44}$,
G.~Chatzikonstantinidis$^{49}$,
M.~Chefdeville$^{6}$,
V.~Chekalina$^{39}$,
C.~Chen$^{3}$,
S.~Chen$^{24}$,
A.~Chernov$^{31}$,
S.-G.~Chitic$^{44}$,
V.~Chobanova$^{43}$,
M.~Chrzaszcz$^{44}$,
A.~Chubykin$^{35}$,
P.~Ciambrone$^{20}$,
M.F.~Cicala$^{52}$,
X.~Cid~Vidal$^{43}$,
G.~Ciezarek$^{44}$,
F.~Cindolo$^{17}$,
P.E.L.~Clarke$^{54}$,
M.~Clemencic$^{44}$,
H.V.~Cliff$^{51}$,
J.~Closier$^{44}$,
J.L.~Cobbledick$^{58}$,
V.~Coco$^{44}$,
J.A.B.~Coelho$^{9}$,
J.~Cogan$^{8}$,
E.~Cogneras$^{7}$,
L.~Cojocariu$^{34}$,
P.~Collins$^{44}$,
T.~Colombo$^{44}$,
A.~Comerma-Montells$^{14}$,
A.~Contu$^{24}$,
N.~Cooke$^{49}$,
G.~Coombs$^{55}$,
S.~Coquereau$^{42}$,
G.~Corti$^{44}$,
C.M.~Costa~Sobral$^{52}$,
B.~Couturier$^{44}$,
G.A.~Cowan$^{54}$,
D.C.~Craik$^{60}$,
A.~Crocombe$^{52}$,
M.~Cruz~Torres$^{1}$,
R.~Currie$^{54}$,
C.L.~Da~Silva$^{63}$,
E.~Dall'Occo$^{29}$,
J.~Dalseno$^{43,w}$,
C.~D'Ambrosio$^{44}$,
A.~Danilina$^{36}$,
P.~d'Argent$^{14}$,
A.~Davis$^{58}$,
O.~De~Aguiar~Francisco$^{44}$,
K.~De~Bruyn$^{44}$,
S.~De~Capua$^{58}$,
M.~De~Cian$^{45}$,
J.M.~De~Miranda$^{1}$,
L.~De~Paula$^{2}$,
M.~De~Serio$^{16,d}$,
P.~De~Simone$^{20}$,
J.A.~de~Vries$^{29}$,
C.T.~Dean$^{63}$,
W.~Dean$^{78}$,
D.~Decamp$^{6}$,
L.~Del~Buono$^{10}$,
B.~Delaney$^{51}$,
H.-P.~Dembinski$^{13}$,
M.~Demmer$^{12}$,
A.~Dendek$^{32}$,
V.~Denysenko$^{46}$,
D.~Derkach$^{75}$,
O.~Deschamps$^{7}$,
F.~Desse$^{9}$,
F.~Dettori$^{24}$,
B.~Dey$^{69}$,
A.~Di~Canto$^{44}$,
P.~Di~Nezza$^{20}$,
S.~Didenko$^{74}$,
H.~Dijkstra$^{44}$,
F.~Dordei$^{24}$,
M.~Dorigo$^{26,z}$,
A.C.~dos~Reis$^{1}$,
A.~Dosil~Su{\'a}rez$^{43}$,
L.~Douglas$^{55}$,
A.~Dovbnya$^{47}$,
K.~Dreimanis$^{56}$,
M.W.~Dudek$^{31}$,
L.~Dufour$^{44}$,
G.~Dujany$^{10}$,
P.~Durante$^{44}$,
J.M.~Durham$^{63}$,
D.~Dutta$^{58}$,
R.~Dzhelyadin$^{41,\dagger}$,
M.~Dziewiecki$^{14}$,
A.~Dziurda$^{31}$,
A.~Dzyuba$^{35}$,
S.~Easo$^{53}$,
U.~Egede$^{57}$,
V.~Egorychev$^{36}$,
S.~Eidelman$^{40,y}$,
S.~Eisenhardt$^{54}$,
R.~Ekelhof$^{12}$,
S.~Ek-In$^{45}$,
L.~Eklund$^{55}$,
S.~Ely$^{64}$,
A.~Ene$^{34}$,
S.~Escher$^{11}$,
S.~Esen$^{29}$,
T.~Evans$^{61}$,
A.~Falabella$^{17}$,
J.~Fan$^{3}$,
N.~Farley$^{49}$,
S.~Farry$^{56}$,
D.~Fazzini$^{9}$,
M.~F{\'e}o$^{44}$,
P.~Fernandez~Declara$^{44}$,
A.~Fernandez~Prieto$^{43}$,
F.~Ferrari$^{17,e}$,
L.~Ferreira~Lopes$^{45}$,
F.~Ferreira~Rodrigues$^{2}$,
S.~Ferreres~Sole$^{29}$,
M.~Ferro-Luzzi$^{44}$,
S.~Filippov$^{38}$,
R.A.~Fini$^{16}$,
M.~Fiorini$^{18,g}$,
M.~Firlej$^{32}$,
K.M.~Fischer$^{59}$,
C.~Fitzpatrick$^{44}$,
T.~Fiutowski$^{32}$,
F.~Fleuret$^{9,b}$,
M.~Fontana$^{44}$,
F.~Fontanelli$^{21,h}$,
R.~Forty$^{44}$,
V.~Franco~Lima$^{56}$,
M.~Franco~Sevilla$^{62}$,
M.~Frank$^{44}$,
C.~Frei$^{44}$,
D.A.~Friday$^{55}$,
J.~Fu$^{23,q}$,
W.~Funk$^{44}$,
E.~Gabriel$^{54}$,
A.~Gallas~Torreira$^{43}$,
D.~Galli$^{17,e}$,
S.~Gallorini$^{25}$,
S.~Gambetta$^{54}$,
Y.~Gan$^{3}$,
M.~Gandelman$^{2}$,
P.~Gandini$^{23}$,
Y.~Gao$^{3}$,
L.M.~Garcia~Martin$^{77}$,
J.~Garc{\'\i}a~Pardi{\~n}as$^{46}$,
B.~Garcia~Plana$^{43}$,
F.A.~Garcia~Rosales$^{9}$,
J.~Garra~Tico$^{51}$,
L.~Garrido$^{42}$,
D.~Gascon$^{42}$,
C.~Gaspar$^{44}$,
G.~Gazzoni$^{7}$,
D.~Gerick$^{14}$,
E.~Gersabeck$^{58}$,
M.~Gersabeck$^{58}$,
T.~Gershon$^{52}$,
D.~Gerstel$^{8}$,
Ph.~Ghez$^{6}$,
V.~Gibson$^{51}$,
A.~Giovent{\`u}$^{43}$,
O.G.~Girard$^{45}$,
P.~Gironella~Gironell$^{42}$,
L.~Giubega$^{34}$,
C.~Giugliano$^{18}$,
K.~Gizdov$^{54}$,
V.V.~Gligorov$^{10}$,
C.~G{\"o}bel$^{66}$,
D.~Golubkov$^{36}$,
A.~Golutvin$^{57,74}$,
A.~Gomes$^{1,a}$,
I.V.~Gorelov$^{37}$,
C.~Gotti$^{22,i}$,
E.~Govorkova$^{29}$,
J.P.~Grabowski$^{14}$,
R.~Graciani~Diaz$^{42}$,
T.~Grammatico$^{10}$,
L.A.~Granado~Cardoso$^{44}$,
E.~Graug{\'e}s$^{42}$,
E.~Graverini$^{45}$,
G.~Graziani$^{19}$,
A.~Grecu$^{34}$,
R.~Greim$^{29}$,
P.~Griffith$^{18}$,
L.~Grillo$^{58}$,
L.~Gruber$^{44}$,
B.R.~Gruberg~Cazon$^{59}$,
C.~Gu$^{3}$,
E.~Gushchin$^{38}$,
A.~Guth$^{11}$,
Yu.~Guz$^{41,44}$,
T.~Gys$^{44}$,
T.~Hadavizadeh$^{59}$,
C.~Hadjivasiliou$^{7}$,
G.~Haefeli$^{45}$,
C.~Haen$^{44}$,
S.C.~Haines$^{51}$,
P.M.~Hamilton$^{62}$,
Q.~Han$^{69}$,
X.~Han$^{14}$,
T.H.~Hancock$^{59}$,
S.~Hansmann-Menzemer$^{14}$,
N.~Harnew$^{59}$,
T.~Harrison$^{56}$,
R.~Hart$^{29}$,
C.~Hasse$^{44}$,
M.~Hatch$^{44}$,
J.~He$^{4}$,
M.~Hecker$^{57}$,
K.~Heijhoff$^{29}$,
K.~Heinicke$^{12}$,
A.~Heister$^{12}$,
A.M.~Hennequin$^{44}$,
K.~Hennessy$^{56}$,
L.~Henry$^{77}$,
M.~He{\ss}$^{71}$,
J.~Heuel$^{11}$,
A.~Hicheur$^{65}$,
R.~Hidalgo~Charman$^{58}$,
D.~Hill$^{59}$,
M.~Hilton$^{58}$,
P.H.~Hopchev$^{45}$,
J.~Hu$^{14}$,
W.~Hu$^{69}$,
W.~Huang$^{4}$,
Z.C.~Huard$^{61}$,
W.~Hulsbergen$^{29}$,
T.~Humair$^{57}$,
R.J.~Hunter$^{52}$,
M.~Hushchyn$^{75}$,
D.~Hutchcroft$^{56}$,
D.~Hynds$^{29}$,
P.~Ibis$^{12}$,
M.~Idzik$^{32}$,
P.~Ilten$^{49}$,
A.~Inglessi$^{35}$,
A.~Inyakin$^{41}$,
K.~Ivshin$^{35}$,
R.~Jacobsson$^{44}$,
S.~Jakobsen$^{44}$,
J.~Jalocha$^{59}$,
E.~Jans$^{29}$,
B.K.~Jashal$^{77}$,
A.~Jawahery$^{62}$,
V.~Jevtic$^{12}$,
F.~Jiang$^{3}$,
M.~John$^{59}$,
D.~Johnson$^{44}$,
C.R.~Jones$^{51}$,
B.~Jost$^{44}$,
N.~Jurik$^{59}$,
S.~Kandybei$^{47}$,
M.~Karacson$^{44}$,
J.M.~Kariuki$^{50}$,
S.~Karodia$^{55}$,
N.~Kazeev$^{75}$,
M.~Kecke$^{14}$,
F.~Keizer$^{51}$,
M.~Kelsey$^{64}$,
M.~Kenzie$^{51}$,
T.~Ketel$^{30}$,
B.~Khanji$^{44}$,
A.~Kharisova$^{76}$,
C.~Khurewathanakul$^{45}$,
K.E.~Kim$^{64}$,
T.~Kirn$^{11}$,
V.S.~Kirsebom$^{45}$,
S.~Klaver$^{20}$,
K.~Klimaszewski$^{33}$,
P.~Kodassery~Padmalayammadam$^{31}$,
S.~Koliiev$^{48}$,
A.~Kondybayeva$^{74}$,
A.~Konoplyannikov$^{36}$,
P.~Kopciewicz$^{32}$,
R.~Kopecna$^{14}$,
P.~Koppenburg$^{29}$,
I.~Kostiuk$^{29,48}$,
O.~Kot$^{48}$,
S.~Kotriakhova$^{35}$,
M.~Kozeiha$^{7}$,
L.~Kravchuk$^{38}$,
R.D.~Krawczyk$^{44}$,
M.~Kreps$^{52}$,
F.~Kress$^{57}$,
S.~Kretzschmar$^{11}$,
P.~Krokovny$^{40,y}$,
W.~Krupa$^{32}$,
W.~Krzemien$^{33}$,
W.~Kucewicz$^{31,l}$,
M.~Kucharczyk$^{31}$,
V.~Kudryavtsev$^{40,y}$,
H.S.~Kuindersma$^{29}$,
G.J.~Kunde$^{63}$,
A.K.~Kuonen$^{45}$,
T.~Kvaratskheliya$^{36}$,
D.~Lacarrere$^{44}$,
G.~Lafferty$^{58}$,
A.~Lai$^{24}$,
D.~Lancierini$^{46}$,
J.J.~Lane$^{58}$,
G.~Lanfranchi$^{20}$,
C.~Langenbruch$^{11}$,
T.~Latham$^{52}$,
F.~Lazzari$^{26,v}$,
C.~Lazzeroni$^{49}$,
R.~Le~Gac$^{8}$,
R.~Lef{\`e}vre$^{7}$,
A.~Leflat$^{37}$,
F.~Lemaitre$^{44}$,
O.~Leroy$^{8}$,
T.~Lesiak$^{31}$,
B.~Leverington$^{14}$,
H.~Li$^{67}$,
P.-R.~Li$^{4,ac}$,
X.~Li$^{63}$,
Y.~Li$^{5}$,
Z.~Li$^{64}$,
X.~Liang$^{64}$,
R.~Lindner$^{44}$,
F.~Lionetto$^{46}$,
V.~Lisovskyi$^{9}$,
G.~Liu$^{67}$,
X.~Liu$^{3}$,
D.~Loh$^{52}$,
A.~Loi$^{24}$,
J.~Lomba~Castro$^{43}$,
I.~Longstaff$^{55}$,
J.H.~Lopes$^{2}$,
G.~Loustau$^{46}$,
G.H.~Lovell$^{51}$,
D.~Lucchesi$^{25,o}$,
M.~Lucio~Martinez$^{29}$,
Y.~Luo$^{3}$,
A.~Lupato$^{25}$,
E.~Luppi$^{18,g}$,
O.~Lupton$^{52}$,
A.~Lusiani$^{26}$,
X.~Lyu$^{4}$,
S.~Maccolini$^{17,e}$,
F.~Machefert$^{9}$,
F.~Maciuc$^{34}$,
V.~Macko$^{45}$,
P.~Mackowiak$^{12}$,
S.~Maddrell-Mander$^{50}$,
L.R.~Madhan~Mohan$^{50}$,
O.~Maev$^{35,44}$,
A.~Maevskiy$^{75}$,
K.~Maguire$^{58}$,
D.~Maisuzenko$^{35}$,
M.W.~Majewski$^{32}$,
S.~Malde$^{59}$,
B.~Malecki$^{44}$,
A.~Malinin$^{73}$,
T.~Maltsev$^{40,y}$,
H.~Malygina$^{14}$,
G.~Manca$^{24,f}$,
G.~Mancinelli$^{8}$,
R.~Manera~Escalero$^{42}$,
D.~Manuzzi$^{17,e}$,
D.~Marangotto$^{23,q}$,
J.~Maratas$^{7,x}$,
J.F.~Marchand$^{6}$,
U.~Marconi$^{17}$,
S.~Mariani$^{19}$,
C.~Marin~Benito$^{9}$,
M.~Marinangeli$^{45}$,
P.~Marino$^{45}$,
J.~Marks$^{14}$,
P.J.~Marshall$^{56}$,
G.~Martellotti$^{28}$,
L.~Martinazzoli$^{44}$,
M.~Martinelli$^{44,22,i}$,
D.~Martinez~Santos$^{43}$,
F.~Martinez~Vidal$^{77}$,
A.~Massafferri$^{1}$,
M.~Materok$^{11}$,
R.~Matev$^{44}$,
A.~Mathad$^{46}$,
Z.~Mathe$^{44}$,
V.~Matiunin$^{36}$,
C.~Matteuzzi$^{22}$,
K.R.~Mattioli$^{78}$,
A.~Mauri$^{46}$,
E.~Maurice$^{9,b}$,
M.~McCann$^{57,44}$,
L.~Mcconnell$^{15}$,
A.~McNab$^{58}$,
R.~McNulty$^{15}$,
J.V.~Mead$^{56}$,
B.~Meadows$^{61}$,
C.~Meaux$^{8}$,
N.~Meinert$^{71}$,
D.~Melnychuk$^{33}$,
S.~Meloni$^{22,i}$,
M.~Merk$^{29}$,
A.~Merli$^{23,q}$,
E.~Michielin$^{25}$,
D.A.~Milanes$^{70}$,
E.~Millard$^{52}$,
M.-N.~Minard$^{6}$,
O.~Mineev$^{36}$,
L.~Minzoni$^{18,g}$,
S.E.~Mitchell$^{54}$,
B.~Mitreska$^{58}$,
D.S.~Mitzel$^{44}$,
A.~M{\"o}dden$^{12}$,
A.~Mogini$^{10}$,
R.D.~Moise$^{57}$,
T.~Momb{\"a}cher$^{12}$,
I.A.~Monroy$^{70}$,
S.~Monteil$^{7}$,
M.~Morandin$^{25}$,
G.~Morello$^{20}$,
M.J.~Morello$^{26,t}$,
J.~Moron$^{32}$,
A.B.~Morris$^{8}$,
A.G.~Morris$^{52}$,
R.~Mountain$^{64}$,
H.~Mu$^{3}$,
F.~Muheim$^{54}$,
M.~Mukherjee$^{69}$,
M.~Mulder$^{29}$,
D.~M{\"u}ller$^{44}$,
J.~M{\"u}ller$^{12}$,
K.~M{\"u}ller$^{46}$,
V.~M{\"u}ller$^{12}$,
C.H.~Murphy$^{59}$,
D.~Murray$^{58}$,
P.~Naik$^{50}$,
T.~Nakada$^{45}$,
R.~Nandakumar$^{53}$,
A.~Nandi$^{59}$,
T.~Nanut$^{45}$,
I.~Nasteva$^{2}$,
M.~Needham$^{54}$,
N.~Neri$^{23,q}$,
S.~Neubert$^{14}$,
N.~Neufeld$^{44}$,
R.~Newcombe$^{57}$,
T.D.~Nguyen$^{45}$,
C.~Nguyen-Mau$^{45,n}$,
E.M.~Niel$^{9}$,
S.~Nieswand$^{11}$,
N.~Nikitin$^{37}$,
N.S.~Nolte$^{44}$,
A.~Oblakowska-Mucha$^{32}$,
V.~Obraztsov$^{41}$,
S.~Ogilvy$^{55}$,
D.P.~O'Hanlon$^{17}$,
R.~Oldeman$^{24,f}$,
C.J.G.~Onderwater$^{72}$,
J. D.~Osborn$^{78}$,
A.~Ossowska$^{31}$,
J.M.~Otalora~Goicochea$^{2}$,
T.~Ovsiannikova$^{36}$,
P.~Owen$^{46}$,
A.~Oyanguren$^{77}$,
P.R.~Pais$^{45}$,
T.~Pajero$^{26,t}$,
A.~Palano$^{16}$,
M.~Palutan$^{20}$,
G.~Panshin$^{76}$,
A.~Papanestis$^{53}$,
M.~Pappagallo$^{54}$,
L.L.~Pappalardo$^{18,g}$,
W.~Parker$^{62}$,
C.~Parkes$^{58,44}$,
G.~Passaleva$^{19,44}$,
A.~Pastore$^{16}$,
M.~Patel$^{57}$,
C.~Patrignani$^{17,e}$,
A.~Pearce$^{44}$,
A.~Pellegrino$^{29}$,
G.~Penso$^{28}$,
M.~Pepe~Altarelli$^{44}$,
S.~Perazzini$^{17}$,
D.~Pereima$^{36}$,
P.~Perret$^{7}$,
L.~Pescatore$^{45}$,
K.~Petridis$^{50}$,
A.~Petrolini$^{21,h}$,
A.~Petrov$^{73}$,
S.~Petrucci$^{54}$,
M.~Petruzzo$^{23,q}$,
B.~Pietrzyk$^{6}$,
G.~Pietrzyk$^{45}$,
M.~Pikies$^{31}$,
M.~Pili$^{59}$,
D.~Pinci$^{28}$,
J.~Pinzino$^{44}$,
F.~Pisani$^{44}$,
A.~Piucci$^{14}$,
V.~Placinta$^{34}$,
S.~Playfer$^{54}$,
J.~Plews$^{49}$,
M.~Plo~Casasus$^{43}$,
F.~Polci$^{10}$,
M.~Poli~Lener$^{20}$,
M.~Poliakova$^{64}$,
A.~Poluektov$^{8}$,
N.~Polukhina$^{74,c}$,
I.~Polyakov$^{64}$,
E.~Polycarpo$^{2}$,
G.J.~Pomery$^{50}$,
S.~Ponce$^{44}$,
A.~Popov$^{41}$,
D.~Popov$^{49}$,
S.~Poslavskii$^{41}$,
L.P.~Promberger$^{44}$,
C.~Prouve$^{43}$,
V.~Pugatch$^{48}$,
A.~Puig~Navarro$^{46}$,
H.~Pullen$^{59}$,
G.~Punzi$^{26,p}$,
W.~Qian$^{4}$,
J.~Qin$^{4}$,
R.~Quagliani$^{10}$,
B.~Quintana$^{7}$,
N.V.~Raab$^{15}$,
B.~Rachwal$^{32}$,
J.H.~Rademacker$^{50}$,
M.~Rama$^{26}$,
M.~Ramos~Pernas$^{43}$,
M.S.~Rangel$^{2}$,
F.~Ratnikov$^{39,75}$,
G.~Raven$^{30}$,
M.~Ravonel~Salzgeber$^{44}$,
M.~Reboud$^{6}$,
F.~Redi$^{45}$,
S.~Reichert$^{12}$,
F.~Reiss$^{10}$,
C.~Remon~Alepuz$^{77}$,
Z.~Ren$^{3}$,
V.~Renaudin$^{59}$,
S.~Ricciardi$^{53}$,
S.~Richards$^{50}$,
K.~Rinnert$^{56}$,
P.~Robbe$^{9}$,
A.~Robert$^{10}$,
A.B.~Rodrigues$^{45}$,
E.~Rodrigues$^{61}$,
J.A.~Rodriguez~Lopez$^{70}$,
M.~Roehrken$^{44}$,
S.~Roiser$^{44}$,
A.~Rollings$^{59}$,
V.~Romanovskiy$^{41}$,
M.~Romero~Lamas$^{43}$,
A.~Romero~Vidal$^{43}$,
J.D.~Roth$^{78}$,
M.~Rotondo$^{20}$,
M.S.~Rudolph$^{64}$,
T.~Ruf$^{44}$,
J.~Ruiz~Vidal$^{77}$,
J.~Ryzka$^{32}$,
J.J.~Saborido~Silva$^{43}$,
N.~Sagidova$^{35}$,
B.~Saitta$^{24,f}$,
C.~Sanchez~Gras$^{29}$,
C.~Sanchez~Mayordomo$^{77}$,
B.~Sanmartin~Sedes$^{43}$,
R.~Santacesaria$^{28}$,
C.~Santamarina~Rios$^{43}$,
P.~Santangelo$^{20}$,
M.~Santimaria$^{20,44}$,
E.~Santovetti$^{27,j}$,
G.~Sarpis$^{58}$,
A.~Sarti$^{20,k}$,
C.~Satriano$^{28,s}$,
A.~Satta$^{27}$,
M.~Saur$^{4}$,
D.~Savrina$^{36,37}$,
L.G.~Scantlebury~Smead$^{59}$,
S.~Schael$^{11}$,
M.~Schellenberg$^{12}$,
M.~Schiller$^{55}$,
H.~Schindler$^{44}$,
M.~Schmelling$^{13}$,
T.~Schmelzer$^{12}$,
B.~Schmidt$^{44}$,
O.~Schneider$^{45}$,
A.~Schopper$^{44}$,
H.F.~Schreiner$^{61}$,
M.~Schubiger$^{29}$,
S.~Schulte$^{45}$,
M.H.~Schune$^{9}$,
R.~Schwemmer$^{44}$,
B.~Sciascia$^{20}$,
A.~Sciubba$^{28,k}$,
S.~Sellam$^{65}$,
A.~Semennikov$^{36}$,
A.~Sergi$^{49,44}$,
N.~Serra$^{46}$,
J.~Serrano$^{8}$,
L.~Sestini$^{25}$,
A.~Seuthe$^{12}$,
P.~Seyfert$^{44}$,
D.M.~Shangase$^{78}$,
M.~Shapkin$^{41}$,
T.~Shears$^{56}$,
L.~Shekhtman$^{40,y}$,
V.~Shevchenko$^{73,74}$,
E.~Shmanin$^{74}$,
J.D.~Shupperd$^{64}$,
B.G.~Siddi$^{18}$,
R.~Silva~Coutinho$^{46}$,
L.~Silva~de~Oliveira$^{2}$,
G.~Simi$^{25,o}$,
S.~Simone$^{16,d}$,
I.~Skiba$^{18}$,
N.~Skidmore$^{14}$,
T.~Skwarnicki$^{64}$,
M.W.~Slater$^{49}$,
J.G.~Smeaton$^{51}$,
E.~Smith$^{11}$,
I.T.~Smith$^{54}$,
M.~Smith$^{57}$,
M.~Soares$^{17}$,
l.~Soares~Lavra$^{1}$,
M.D.~Sokoloff$^{61}$,
F.J.P.~Soler$^{55}$,
B.~Souza~De~Paula$^{2}$,
B.~Spaan$^{12}$,
E.~Spadaro~Norella$^{23,q}$,
P.~Spradlin$^{55}$,
F.~Stagni$^{44}$,
M.~Stahl$^{61}$,
S.~Stahl$^{44}$,
P.~Stefko$^{45}$,
S.~Stefkova$^{57}$,
O.~Steinkamp$^{46}$,
S.~Stemmle$^{14}$,
O.~Stenyakin$^{41}$,
M.~Stepanova$^{35}$,
H.~Stevens$^{12}$,
A.~Stocchi$^{9}$,
S.~Stone$^{64}$,
S.~Stracka$^{26}$,
M.E.~Stramaglia$^{45}$,
M.~Straticiuc$^{34}$,
U.~Straumann$^{46}$,
S.~Strokov$^{76}$,
J.~Sun$^{3}$,
L.~Sun$^{68}$,
Y.~Sun$^{62}$,
P.~Svihra$^{58}$,
K.~Swientek$^{32}$,
A.~Szabelski$^{33}$,
T.~Szumlak$^{32}$,
M.~Szymanski$^{4}$,
S.~Taneja$^{58}$,
Z.~Tang$^{3}$,
T.~Tekampe$^{12}$,
G.~Tellarini$^{18}$,
F.~Teubert$^{44}$,
E.~Thomas$^{44}$,
K.A.~Thomson$^{56}$,
M.J.~Tilley$^{57}$,
V.~Tisserand$^{7}$,
S.~T'Jampens$^{6}$,
M.~Tobin$^{5}$,
S.~Tolk$^{44}$,
L.~Tomassetti$^{18,g}$,
D.~Tonelli$^{26}$,
D.Y.~Tou$^{10}$,
E.~Tournefier$^{6}$,
M.~Traill$^{55}$,
M.T.~Tran$^{45}$,
A.~Trisovic$^{51}$,
A.~Tsaregorodtsev$^{8}$,
G.~Tuci$^{26,44,p}$,
A.~Tully$^{51}$,
N.~Tuning$^{29}$,
A.~Ukleja$^{33}$,
A.~Usachov$^{9}$,
A.~Ustyuzhanin$^{39,75}$,
U.~Uwer$^{14}$,
A.~Vagner$^{76}$,
V.~Vagnoni$^{17}$,
A.~Valassi$^{44}$,
S.~Valat$^{44}$,
G.~Valenti$^{17}$,
M.~van~Beuzekom$^{29}$,
H.~Van~Hecke$^{63}$,
E.~van~Herwijnen$^{44}$,
C.B.~Van~Hulse$^{15}$,
J.~van~Tilburg$^{29}$,
M.~van~Veghel$^{72}$,
R.~Vazquez~Gomez$^{44}$,
P.~Vazquez~Regueiro$^{43}$,
C.~V{\'a}zquez~Sierra$^{29}$,
S.~Vecchi$^{18}$,
J.J.~Velthuis$^{50}$,
M.~Veltri$^{19,r}$,
A.~Venkateswaran$^{64}$,
M.~Vernet$^{7}$,
M.~Veronesi$^{29}$,
M.~Vesterinen$^{52}$,
J.V.~Viana~Barbosa$^{44}$,
D.~Vieira$^{4}$,
M.~Vieites~Diaz$^{45}$,
H.~Viemann$^{71}$,
X.~Vilasis-Cardona$^{42,m}$,
A.~Vitkovskiy$^{29}$,
V.~Volkov$^{37}$,
A.~Vollhardt$^{46}$,
D.~Vom~Bruch$^{10}$,
B.~Voneki$^{44}$,
A.~Vorobyev$^{35}$,
V.~Vorobyev$^{40,y}$,
N.~Voropaev$^{35}$,
R.~Waldi$^{71}$,
J.~Walsh$^{26}$,
J.~Wang$^{3}$,
J.~Wang$^{5}$,
M.~Wang$^{3}$,
Y.~Wang$^{69}$,
Z.~Wang$^{46}$,
D.R.~Ward$^{51}$,
H.M.~Wark$^{56}$,
N.K.~Watson$^{49}$,
D.~Websdale$^{57}$,
A.~Weiden$^{46}$,
C.~Weisser$^{60}$,
B.D.C.~Westhenry$^{50}$,
D.J.~White$^{58}$,
M.~Whitehead$^{11}$,
D.~Wiedner$^{12}$,
G.~Wilkinson$^{59}$,
M.~Wilkinson$^{64}$,
I.~Williams$^{51}$,
M.~Williams$^{60}$,
M.R.J.~Williams$^{58}$,
T.~Williams$^{49}$,
F.F.~Wilson$^{53}$,
M.~Winn$^{9}$,
W.~Wislicki$^{33}$,
M.~Witek$^{31}$,
G.~Wormser$^{9}$,
S.A.~Wotton$^{51}$,
H.~Wu$^{64}$,
K.~Wyllie$^{44}$,
Z.~Xiang$^{4}$,
D.~Xiao$^{69}$,
Y.~Xie$^{69}$,
H.~Xing$^{67}$,
A.~Xu$^{3}$,
L.~Xu$^{3}$,
M.~Xu$^{69}$,
Q.~Xu$^{4}$,
Z.~Xu$^{6}$,
Z.~Xu$^{3}$,
Z.~Yang$^{3}$,
Z.~Yang$^{62}$,
Y.~Yao$^{64}$,
L.E.~Yeomans$^{56}$,
H.~Yin$^{69}$,
J.~Yu$^{69,ab}$,
X.~Yuan$^{64}$,
O.~Yushchenko$^{41}$,
K.A.~Zarebski$^{49}$,
M.~Zavertyaev$^{13,c}$,
M.~Zdybal$^{31}$,
M.~Zeng$^{3}$,
D.~Zhang$^{69}$,
L.~Zhang$^{3}$,
S.~Zhang$^{3}$,
W.C.~Zhang$^{3,aa}$,
Y.~Zhang$^{44}$,
A.~Zhelezov$^{14}$,
Y.~Zheng$^{4}$,
X.~Zhou$^{4}$,
Y.~Zhou$^{4}$,
X.~Zhu$^{3}$,
V.~Zhukov$^{11,37}$,
J.B.~Zonneveld$^{54}$,
S.~Zucchelli$^{17,e}$.\bigskip

{\footnotesize \it

$ ^{1}$Centro Brasileiro de Pesquisas F{\'\i}sicas (CBPF), Rio de Janeiro, Brazil\\
$ ^{2}$Universidade Federal do Rio de Janeiro (UFRJ), Rio de Janeiro, Brazil\\
$ ^{3}$Center for High Energy Physics, Tsinghua University, Beijing, China\\
$ ^{4}$University of Chinese Academy of Sciences, Beijing, China\\
$ ^{5}$Institute Of High Energy Physics (ihep), Beijing, China\\
$ ^{6}$Univ. Grenoble Alpes, Univ. Savoie Mont Blanc, CNRS, IN2P3-LAPP, Annecy, France\\
$ ^{7}$Universit{\'e} Clermont Auvergne, CNRS/IN2P3, LPC, Clermont-Ferrand, France\\
$ ^{8}$Aix Marseille Univ, CNRS/IN2P3, CPPM, Marseille, France\\
$ ^{9}$LAL, Univ. Paris-Sud, CNRS/IN2P3, Universit{\'e} Paris-Saclay, Orsay, France\\
$ ^{10}$LPNHE, Sorbonne Universit{\'e}, Paris Diderot Sorbonne Paris Cit{\'e}, CNRS/IN2P3, Paris, France\\
$ ^{11}$I. Physikalisches Institut, RWTH Aachen University, Aachen, Germany\\
$ ^{12}$Fakult{\"a}t Physik, Technische Universit{\"a}t Dortmund, Dortmund, Germany\\
$ ^{13}$Max-Planck-Institut f{\"u}r Kernphysik (MPIK), Heidelberg, Germany\\
$ ^{14}$Physikalisches Institut, Ruprecht-Karls-Universit{\"a}t Heidelberg, Heidelberg, Germany\\
$ ^{15}$School of Physics, University College Dublin, Dublin, Ireland\\
$ ^{16}$INFN Sezione di Bari, Bari, Italy\\
$ ^{17}$INFN Sezione di Bologna, Bologna, Italy\\
$ ^{18}$INFN Sezione di Ferrara, Ferrara, Italy\\
$ ^{19}$INFN Sezione di Firenze, Firenze, Italy\\
$ ^{20}$INFN Laboratori Nazionali di Frascati, Frascati, Italy\\
$ ^{21}$INFN Sezione di Genova, Genova, Italy\\
$ ^{22}$INFN Sezione di Milano-Bicocca, Milano, Italy\\
$ ^{23}$INFN Sezione di Milano, Milano, Italy\\
$ ^{24}$INFN Sezione di Cagliari, Monserrato, Italy\\
$ ^{25}$INFN Sezione di Padova, Padova, Italy\\
$ ^{26}$INFN Sezione di Pisa, Pisa, Italy\\
$ ^{27}$INFN Sezione di Roma Tor Vergata, Roma, Italy\\
$ ^{28}$INFN Sezione di Roma La Sapienza, Roma, Italy\\
$ ^{29}$Nikhef National Institute for Subatomic Physics, Amsterdam, Netherlands\\
$ ^{30}$Nikhef National Institute for Subatomic Physics and VU University Amsterdam, Amsterdam, Netherlands\\
$ ^{31}$Henryk Niewodniczanski Institute of Nuclear Physics  Polish Academy of Sciences, Krak{\'o}w, Poland\\
$ ^{32}$AGH - University of Science and Technology, Faculty of Physics and Applied Computer Science, Krak{\'o}w, Poland\\
$ ^{33}$National Center for Nuclear Research (NCBJ), Warsaw, Poland\\
$ ^{34}$Horia Hulubei National Institute of Physics and Nuclear Engineering, Bucharest-Magurele, Romania\\
$ ^{35}$Petersburg Nuclear Physics Institute NRC Kurchatov Institute (PNPI NRC KI), Gatchina, Russia\\
$ ^{36}$Institute of Theoretical and Experimental Physics NRC Kurchatov Institute (ITEP NRC KI), Moscow, Russia, Moscow, Russia\\
$ ^{37}$Institute of Nuclear Physics, Moscow State University (SINP MSU), Moscow, Russia\\
$ ^{38}$Institute for Nuclear Research of the Russian Academy of Sciences (INR RAS), Moscow, Russia\\
$ ^{39}$Yandex School of Data Analysis, Moscow, Russia\\
$ ^{40}$Budker Institute of Nuclear Physics (SB RAS), Novosibirsk, Russia\\
$ ^{41}$Institute for High Energy Physics NRC Kurchatov Institute (IHEP NRC KI), Protvino, Russia, Protvino, Russia\\
$ ^{42}$ICCUB, Universitat de Barcelona, Barcelona, Spain\\
$ ^{43}$Instituto Galego de F{\'\i}sica de Altas Enerx{\'\i}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain\\
$ ^{44}$European Organization for Nuclear Research (CERN), Geneva, Switzerland\\
$ ^{45}$Institute of Physics, Ecole Polytechnique  F{\'e}d{\'e}rale de Lausanne (EPFL), Lausanne, Switzerland\\
$ ^{46}$Physik-Institut, Universit{\"a}t Z{\"u}rich, Z{\"u}rich, Switzerland\\
$ ^{47}$NSC Kharkiv Institute of Physics and Technology (NSC KIPT), Kharkiv, Ukraine\\
$ ^{48}$Institute for Nuclear Research of the National Academy of Sciences (KINR), Kyiv, Ukraine\\
$ ^{49}$University of Birmingham, Birmingham, United Kingdom\\
$ ^{50}$H.H. Wills Physics Laboratory, University of Bristol, Bristol, United Kingdom\\
$ ^{51}$Cavendish Laboratory, University of Cambridge, Cambridge, United Kingdom\\
$ ^{52}$Department of Physics, University of Warwick, Coventry, United Kingdom\\
$ ^{53}$STFC Rutherford Appleton Laboratory, Didcot, United Kingdom\\
$ ^{54}$School of Physics and Astronomy, University of Edinburgh, Edinburgh, United Kingdom\\
$ ^{55}$School of Physics and Astronomy, University of Glasgow, Glasgow, United Kingdom\\
$ ^{56}$Oliver Lodge Laboratory, University of Liverpool, Liverpool, United Kingdom\\
$ ^{57}$Imperial College London, London, United Kingdom\\
$ ^{58}$School of Physics and Astronomy, University of Manchester, Manchester, United Kingdom\\
$ ^{59}$Department of Physics, University of Oxford, Oxford, United Kingdom\\
$ ^{60}$Massachusetts Institute of Technology, Cambridge, MA, United States\\
$ ^{61}$University of Cincinnati, Cincinnati, OH, United States\\
$ ^{62}$University of Maryland, College Park, MD, United States\\
$ ^{63}$Los Alamos National Laboratory (LANL), Los Alamos, United States\\
$ ^{64}$Syracuse University, Syracuse, NY, United States\\
$ ^{65}$Laboratory of Mathematical and Subatomic Physics , Constantine, Algeria, associated to $^{2}$\\
$ ^{66}$Pontif{\'\i}cia Universidade Cat{\'o}lica do Rio de Janeiro (PUC-Rio), Rio de Janeiro, Brazil, associated to $^{2}$\\
$ ^{67}$South China Normal University, Guangzhou, China, associated to $^{3}$\\
$ ^{68}$School of Physics and Technology, Wuhan University, Wuhan, China, associated to $^{3}$\\
$ ^{69}$Institute of Particle Physics, Central China Normal University, Wuhan, Hubei, China, associated to $^{3}$\\
$ ^{70}$Departamento de Fisica , Universidad Nacional de Colombia, Bogota, Colombia, associated to $^{10}$\\
$ ^{71}$Institut f{\"u}r Physik, Universit{\"a}t Rostock, Rostock, Germany, associated to $^{14}$\\
$ ^{72}$Van Swinderen Institute, University of Groningen, Groningen, Netherlands, associated to $^{29}$\\
$ ^{73}$National Research Centre Kurchatov Institute, Moscow, Russia, associated to $^{36}$\\
$ ^{74}$National University of Science and Technology ``MISIS'', Moscow, Russia, associated to $^{36}$\\
$ ^{75}$National Research University Higher School of Economics, Moscow, Russia, associated to $^{39}$\\
$ ^{76}$National Research Tomsk Polytechnic University, Tomsk, Russia, associated to $^{36}$\\
$ ^{77}$Instituto de Fisica Corpuscular, Centro Mixto Universidad de Valencia - CSIC, Valencia, Spain, associated to $^{42}$\\
$ ^{78}$University of Michigan, Ann Arbor, United States, associated to $^{64}$\\
\bigskip
$^{a}$Universidade Federal do Tri{\^a}ngulo Mineiro (UFTM), Uberaba-MG, Brazil\\
$^{b}$Laboratoire Leprince-Ringuet, Palaiseau, France\\
$^{c}$P.N. Lebedev Physical Institute, Russian Academy of Science (LPI RAS), Moscow, Russia\\
$^{d}$Universit{\`a} di Bari, Bari, Italy\\
$^{e}$Universit{\`a} di Bologna, Bologna, Italy\\
$^{f}$Universit{\`a} di Cagliari, Cagliari, Italy\\
$^{g}$Universit{\`a} di Ferrara, Ferrara, Italy\\
$^{h}$Universit{\`a} di Genova, Genova, Italy\\
$^{i}$Universit{\`a} di Milano Bicocca, Milano, Italy\\
$^{j}$Universit{\`a} di Roma Tor Vergata, Roma, Italy\\
$^{k}$Universit{\`a} di Roma La Sapienza, Roma, Italy\\
$^{l}$AGH - University of Science and Technology, Faculty of Computer Science, Electronics and Telecommunications, Krak{\'o}w, Poland\\
$^{m}$LIFAELS, La Salle, Universitat Ramon Llull, Barcelona, Spain\\
$^{n}$Hanoi University of Science, Hanoi, Vietnam\\
$^{o}$Universit{\`a} di Padova, Padova, Italy\\
$^{p}$Universit{\`a} di Pisa, Pisa, Italy\\
$^{q}$Universit{\`a} degli Studi di Milano, Milano, Italy\\
$^{r}$Universit{\`a} di Urbino, Urbino, Italy\\
$^{s}$Universit{\`a} della Basilicata, Potenza, Italy\\
$^{t}$Scuola Normale Superiore, Pisa, Italy\\
$^{u}$Universit{\`a} di Modena e Reggio Emilia, Modena, Italy\\
$^{v}$Universit{\`a} di Siena, Siena, Italy\\
$^{w}$H.H. Wills Physics Laboratory, University of Bristol, Bristol, United Kingdom\\
$^{x}$MSU - Iligan Institute of Technology (MSU-IIT), Iligan, Philippines\\
$^{y}$Novosibirsk State University, Novosibirsk, Russia\\
$^{z}$Sezione INFN di Trieste, Trieste, Italy\\
$^{aa}$School of Physics and Information Technology, Shaanxi Normal University (SNNU), Xi'an, China\\
$^{ab}$Physics and Micro Electronic College, Hunan University, Changsha City, China\\
$^{ac}$Lanzhou University, Lanzhou, China\\
\medskip
$ ^{\dagger}$Deceased
}
\end{flushleft}

==> LHCb_Authorship_flat_arXiv_11-Jun-2019.tex <==
LHCb collaboration: 
R. Aaij,
C. Abell{\'a}n Beteta,
T. Ackernley,
B. Adeva,
M. Adinolfi,
H. Afsharnia,
C.A. Aidala,
S. Aiola,
Z. Ajaltouni,
S. Akar,
P. Albicocco,
J. Albrecht,
F. Alessio,
M. Alexander,
A. Alfonso Albero,
G. Alkhazov,
P. Alvarez Cartelle,
A.A. Alves Jr,
S. Amato,
Y. Amhis,
L. An,
L. Anderlini,
G. Andreassi,
M. Andreotti,
F. Archilli,
P. d'Argent,
J. Arnau Romeu,
A. Artamonov,
M. Artuso,
K. Arzymatov,
E. Aslanides,
M. Atzeni,
B. Audurier,
S. Bachmann,
J.J. Back,
S. Baker,
V. Balagura,
W. Baldini,
A. Baranov,
R.J. Barlow,
S. Barsuk,
W. Barter,
M. Bartolini,
F. Baryshnikov,
G. Bassi,
V. Batozskaya,
B. Batsukh,
A. Battig,
V. Battista,
A. Bay,
M. Becker,
F. Bedeschi,
I. Bediaga,
A. Beiter,
L.J. Bel,
V. Belavin,
S. Belin,
N. Beliy,
V. Bellee,
K. Belous,
I. Belyaev,
E. Ben-Haim,
G. Bencivenni,
S. Benson,
S. Beranek,
A. Berezhnoy,
R. Bernet,
D. Berninghoff,
H.C. Bernstein,
E. Bertholet,
A. Bertolin,
C. Betancourt,
F. Betti,
M.O. Bettler,
M. van Beuzekom,
Ia. Bezshyiko,
S. Bhasin,
J. Bhom,
M.S. Bieker,
S. Bifani,
P. Billoir,
A. Birnkraut,
A. Bizzeti,
M. Bj{\o}rn,
M.P. Blago,
T. Blake,
F. Blanc,
S. Blusk,
D. Bobulska,
V. Bocci,
O. Boente Garcia,
T. Boettcher,
A. Boldyrev,
A. Bondar,
N. Bondar,
S. Borghi,
M. Borisyak,
M. Borsato,
J.T. Borsuk,
M. Boubdir,
T.J.V. Bowcock,
C. Bozzi,
S. Braun,
A. Brea Rodriguez,
M. Brodski,
J. Brodzicka,
A. Brossa Gonzalo,
D. Brundu,
E. Buchanan,
A. Buonaura,
C. Burr,
A. Bursche,
J.S. Butter,
J. Buytaert,
W. Byczynski,
S. Cadeddu,
H. Cai,
R. Calabrese,
S. Cali,
R. Calladine,
M. Calvi,
M. Calvo Gomez,
A. Camboni,
P. Campana,
D.H. Campora Perez,
L. Capriotti,
A. Carbone,
G. Carboni,
R. Cardinale,
A. Cardini,
P. Carniti,
K. Carvalho Akiba,
A. Casais Vidal,
G. Casse,
M. Cattaneo,
G. Cavallero,
R. Cenci,
J. Cerasoli,
M.G. Chapman,
M. Charles,
Ph. Charpentier,
G. Chatzikonstantinidis,
M. Chefdeville,
V. Chekalina,
C. Chen,
S. Chen,
A. Chernov,
S.-G. Chitic,
V. Chobanova,
M. Chrzaszcz,
A. Chubykin,
P. Ciambrone,
M.F. Cicala,
X. Cid Vidal,
G. Ciezarek,
F. Cindolo,
P.E.L. Clarke,
M. Clemencic,
H.V. Cliff,
J. Closier,
J.L. Cobbledick,
V. Coco,
J.A.B. Coelho,
J. Cogan,
E. Cogneras,
L. Cojocariu,
P. Collins,
T. Colombo,
A. Comerma-Montells,
A. Contu,
N. Cooke,
G. Coombs,
S. Coquereau,
G. Corti,
C.M. Costa Sobral,
B. Couturier,
G.A. Cowan,
D.C. Craik,
A. Crocombe,
M. Cruz Torres,
R. Currie,
C. D'Ambrosio,
C.L. Da Silva,
E. Dall'Occo,
J. Dalseno,
A. Danilina,
A. Davis,
O. De Aguiar Francisco,
K. De Bruyn,
S. De Capua,
M. De Cian,
J.M. De Miranda,
L. De Paula,
M. De Serio,
P. De Simone,
C.T. Dean,
W. Dean,
D. Decamp,
L. Del Buono,
B. Delaney,
H.-P. Dembinski,
M. Demmer,
A. Dendek,
V. Denysenko,
D. Derkach,
O. Deschamps,
F. Desse,
F. Dettori,
B. Dey,
A. Di Canto,
P. Di Nezza,
S. Didenko,
H. Dijkstra,
F. Dordei,
M. Dorigo,
A. Dosil Su{\'a}rez,
L. Douglas,
A. Dovbnya,
K. Dreimanis,
M.W. Dudek,
L. Dufour,
G. Dujany,
P. Durante,
J.M. Durham,
D. Dutta,
R. Dzhelyadin,
M. Dziewiecki,
A. Dziurda,
A. Dzyuba,
S. Easo,
U. Egede,
V. Egorychev,
S. Eidelman,
S. Eisenhardt,
S. Ek-In,
R. Ekelhof,
L. Eklund,
S. Ely,
A. Ene,
S. Escher,
S. Esen,
T. Evans,
A. Falabella,
J. Fan,
N. Farley,
S. Farry,
D. Fazzini,
P. Fernandez Declara,
A. Fernandez Prieto,
F. Ferrari,
L. Ferreira Lopes,
F. Ferreira Rodrigues,
S. Ferreres Sole,
M. Ferro-Luzzi,
S. Filippov,
R.A. Fini,
M. Fiorini,
M. Firlej,
K.M. Fischer,
C. Fitzpatrick,
T. Fiutowski,
F. Fleuret,
M. Fontana,
F. Fontanelli,
R. Forty,
V. Franco Lima,
M. Franco Sevilla,
M. Frank,
C. Frei,
D.A. Friday,
J. Fu,
W. Funk,
M. F{\'e}o,
E. Gabriel,
A. Gallas Torreira,
D. Galli,
S. Gallorini,
S. Gambetta,
Y. Gan,
M. Gandelman,
P. Gandini,
Y. Gao,
L.M. Garcia Martin,
B. Garcia Plana,
F.A. Garcia Rosales,
J. Garc{\'\i}a Pardi{\~n}as,
J. Garra Tico,
L. Garrido,
D. Gascon,
C. Gaspar,
G. Gazzoni,
D. Gerick,
E. Gersabeck,
M. Gersabeck,
T. Gershon,
D. Gerstel,
Ph. Ghez,
V. Gibson,
A. Giovent{\`u},
O.G. Girard,
P. Gironella Gironell,
L. Giubega,
C. Giugliano,
K. Gizdov,
V.V. Gligorov,
D. Golubkov,
A. Golutvin,
A. Gomes,
I.V. Gorelov,
C. Gotti,
E. Govorkova,
J.P. Grabowski,
R. Graciani Diaz,
T. Grammatico,
L.A. Granado Cardoso,
E. Graug{\'e}s,
E. Graverini,
G. Graziani,
A. Grecu,
R. Greim,
P. Griffith,
L. Grillo,
L. Gruber,
B.R. Gruberg Cazon,
C. Gu,
X. Guo,
E. Gushchin,
A. Guth,
Yu. Guz,
T. Gys,
C. G{\"o}bel,
T. Hadavizadeh,
C. Hadjivasiliou,
G. Haefeli,
C. Haen,
S.C. Haines,
P.M. Hamilton,
Q. Han,
X. Han,
T.H. Hancock,
S. Hansmann-Menzemer,
N. Harnew,
T. Harrison,
R. Hart,
C. Hasse,
M. Hatch,
J. He,
M. Hecker,
K. Heijhoff,
K. Heinicke,
A. Heister,
A.M. Hennequin,
K. Hennessy,
L. Henry,
E. van Herwijnen,
J. Heuel,
M. He{\ss},
A. Hicheur,
R. Hidalgo Charman,
D. Hill,
M. Hilton,
P.H. Hopchev,
J. Hu,
W. Hu,
W. Huang,
Z.C. Huard,
W. Hulsbergen,
T. Humair,
R.J. Hunter,
M. Hushchyn,
D. Hutchcroft,
D. Hynds,
P. Ibis,
M. Idzik,
P. Ilten,
A. Inglessi,
A. Inyakin,
K. Ivshin,
R. Jacobsson,
S. Jakobsen,
J. Jalocha,
E. Jans,
B.K. Jashal,
A. Jawahery,
V. Jevtic,
F. Jiang,
M. John,
D. Johnson,
C.R. Jones,
B. Jost,
N. Jurik,
S. Kandybei,
M. Karacson,
J.M. Kariuki,
S. Karodia,
N. Kazeev,
M. Kecke,
F. Keizer,
M. Kelsey,
M. Kenzie,
T. Ketel,
B. Khanji,
A. Kharisova,
C. Khurewathanakul,
K.E. Kim,
T. Kirn,
V.S. Kirsebom,
S. Klaver,
K. Klimaszewski,
S. Koliiev,
A. Kondybayeva,
A. Konoplyannikov,
P. Kopciewicz,
R. Kopecna,
P. Koppenburg,
I. Kostiuk,
O. Kot,
S. Kotriakhova,
M. Kozeiha,
L. Kravchuk,
R.D. Krawczyk,
M. Kreps,
F. Kress,
S. Kretzschmar,
P. Krokovny,
W. Krupa,
W. Krzemien,
W. Kucewicz,
M. Kucharczyk,
V. Kudryavtsev,
H.S. Kuindersma,
G.J. Kunde,
A.K. Kuonen,
T. Kvaratskheliya,
D. Lacarrere,
G. Lafferty,
A. Lai,
D. Lancierini,
J.J. Lane,
G. Lanfranchi,
C. Langenbruch,
T. Latham,
F. Lazzari,
C. Lazzeroni,
R. Le Gac,
A. Leflat,
R. Lef{\`e}vre,
F. Lemaitre,
O. Leroy,
T. Lesiak,
B. Leverington,
H. Li,
P.-R. Li,
X. Li,
Y. Li,
Z. Li,
X. Liang,
R. Lindner,
P. Ling,
F. Lionetto,
V. Lisovskyi,
G. Liu,
X. Liu,
D. Loh,
A. Loi,
J. Lomba Castro,
I. Longstaff,
J.H. Lopes,
G. Loustau,
G.H. Lovell,
D. Lucchesi,
M. Lucio Martinez,
Y. Luo,
A. Lupato,
E. Luppi,
O. Lupton,
A. Lusiani,
X. Lyu,
R. Ma,
S. Maccolini,
F. Machefert,
F. Maciuc,
V. Macko,
P. Mackowiak,
S. Maddrell-Mander,
L.R. Madhan Mohan,
O. Maev,
A. Maevskiy,
K. Maguire,
D. Maisuzenko,
M.W. Majewski,
S. Malde,
B. Malecki,
A. Malinin,
T. Maltsev,
H. Malygina,
G. Manca,
G. Mancinelli,
R. Manera Escalero,
D. Manuzzi,
D. Marangotto,
J. Maratas,
J.F. Marchand,
U. Marconi,
S. Mariani,
C. Marin Benito,
M. Marinangeli,
P. Marino,
J. Marks,
P.J. Marshall,
G. Martellotti,
L. Martinazzoli,
M. Martinelli,
D. Martinez Santos,
F. Martinez Vidal,
A. Massafferri,
M. Materok,
R. Matev,
A. Mathad,
Z. Mathe,
V. Matiunin,
C. Matteuzzi,
K.R. Mattioli,
A. Mauri,
E. Maurice,
M. McCann,
L. Mcconnell,
A. McNab,
R. McNulty,
J.V. Mead,
B. Meadows,
C. Meaux,
N. Meinert,
D. Melnychuk,
S. Meloni,
M. Merk,
A. Merli,
E. Michielin,
D.A. Milanes,
E. Millard,
M.-N. Minard,
O. Mineev,
L. Minzoni,
S.E. Mitchell,
B. Mitreska,
D.S. Mitzel,
A. Mogini,
R.D. Moise,
T. Momb{\"a}cher,
I.A. Monroy,
S. Monteil,
M. Morandin,
G. Morello,
M.J. Morello,
J. Moron,
A.B. Morris,
A.G. Morris,
R. Mountain,
H. Mu,
F. Muheim,
M. Mukherjee,
M. Mulder,
C.H. Murphy,
D. Murray,
P. Muzzetto,
A. M{\"o}dden ,
D. M{\"u}ller,
J. M{\"u}ller,
K. M{\"u}ller,
V. M{\"u}ller,
P. Naik,
T. Nakada,
R. Nandakumar,
A. Nandi,
T. Nanut,
I. Nasteva,
M. Needham,
N. Neri,
S. Neubert,
N. Neufeld,
R. Newcombe,
T.D. Nguyen,
C. Nguyen-Mau,
E.M. Niel,
S. Nieswand,
N. Nikitin,
N.S. Nolte,
D.P. O'Hanlon,
A. Oblakowska-Mucha,
V. Obraztsov,
S. Ogilvy,
R. Oldeman,
C.J.G. Onderwater,
J. D. Osborn,
A. Ossowska,
J.M. Otalora Goicochea,
T. Ovsiannikova,
P. Owen,
A. Oyanguren,
P.R. Pais,
T. Pajero,
A. Palano,
M. Palutan,
G. Panshin,
A. Papanestis,
M. Pappagallo,
L.L. Pappalardo,
W. Parker,
C. Parkes,
G. Passaleva,
A. Pastore,
M. Patel,
C. Patrignani,
A. Pearce,
A. Pellegrino,
G. Penso,
M. Pepe Altarelli,
S. Perazzini,
D. Pereima,
P. Perret,
L. Pescatore,
K. Petridis,
A. Petrolini,
A. Petrov,
S. Petrucci,
M. Petruzzo,
B. Pietrzyk,
G. Pietrzyk,
M. Pikies,
M. Pili,
D. Pinci,
J. Pinzino,
F. Pisani,
A. Piucci,
V. Placinta,
S. Playfer,
J. Plews,
M. Plo Casasus,
F. Polci,
M. Poli Lener,
M. Poliakova,
A. Poluektov,
N. Polukhina,
I. Polyakov,
E. Polycarpo,
G.J. Pomery,
S. Ponce,
A. Popov,
D. Popov,
S. Poslavskii,
K. Prasanth,
L. Promberger,
C. Prouve,
V. Pugatch,
A. Puig Navarro,
H. Pullen,
G. Punzi,
W. Qian,
J. Qin,
R. Quagliani,
B. Quintana,
N.V. Raab,
B. Rachwal,
J.H. Rademacker,
M. Rama,
M. Ramos Pernas,
M.S. Rangel,
F. Ratnikov,
G. Raven,
M. Ravonel Salzgeber,
M. Reboud,
F. Redi,
S. Reichert,
A.C. dos Reis,
F. Reiss,
C. Remon Alepuz,
Z. Ren,
V. Renaudin,
S. Ricciardi,
S. Richards,
K. Rinnert,
P. Robbe,
A. Robert,
A.B. Rodrigues,
E. Rodrigues,
J.A. Rodriguez Lopez,
M. Roehrken,
S. Roiser,
A. Rollings,
V. Romanovskiy,
M. Romero Lamas,
A. Romero Vidal,
J.D. Roth,
M. Rotondo,
M.S. Rudolph,
T. Ruf,
J. Ruiz Vidal,
J. Ryzka,
J.J. Saborido Silva,
N. Sagidova,
B. Saitta,
C. Sanchez Gras,
C. Sanchez Mayordomo,
B. Sanmartin Sedes,
R. Santacesaria,
C. Santamarina Rios,
M. Santimaria,
E. Santovetti,
G. Sarpis,
A. Sarti,
C. Satriano,
A. Satta,
M. Saur,
D. Savrina,
L.G. Scantlebury Smead,
S. Schael,
M. Schellenberg,
M. Schiller,
H. Schindler,
M. Schmelling,
T. Schmelzer,
B. Schmidt,
O. Schneider,
A. Schopper,
H.F. Schreiner,
M. Schubiger,
S. Schulte,
M.H. Schune,
R. Schwemmer,
B. Sciascia,
A. Sciubba,
S. Sellam,
A. Semennikov,
A. Sergi,
N. Serra,
J. Serrano,
L. Sestini,
A. Seuthe,
P. Seyfert,
D.M. Shangase,
M. Shapkin,
T. Shears,
L. Shekhtman,
V. Shevchenko,
E. Shmanin,
J.D. Shupperd,
B.G. Siddi,
R. Silva Coutinho,
L. Silva de Oliveira,
G. Simi,
S. Simone,
I. Skiba,
N. Skidmore,
T. Skwarnicki,
M.W. Slater,
J.G. Smeaton,
E. Smith,
I.T. Smith,
M. Smith,
M. Soares,
L. Soares Lavra,
M.D. Sokoloff,
F.J.P. Soler,
B. Souza De Paula,
B. Spaan,
E. Spadaro Norella,
P. Spradlin,
F. Stagni,
M. Stahl,
S. Stahl,
P. Stefko,
S. Stefkova,
O. Steinkamp,
S. Stemmle,
O. Stenyakin,
M. Stepanova,
H. Stevens,
S. Stone,
S. Stracka,
M.E. Stramaglia,
M. Straticiuc,
U. Straumann,
S. Strokov,
J. Sun,
L. Sun,
Y. Sun,
P. Svihra,
K. Swientek,
A. Szabelski,
T. Szumlak,
M. Szymanski,
S. T'Jampens,
S. Taneja,
Z. Tang,
T. Tekampe,
G. Tellarini,
F. Teubert,
E. Thomas,
K.A. Thomson,
J. van Tilburg,
M.J. Tilley,
V. Tisserand,
M. Tobin,
S. Tolk,
L. Tomassetti,
D. Tonelli,
D.Y. Tou,
E. Tournefier,
M. Traill,
M.T. Tran,
A. Trisovic,
A. Tsaregorodtsev,
G. Tuci,
A. Tully,
N. Tuning,
A. Ukleja,
A. Usachov,
A. Ustyuzhanin,
U. Uwer,
A. Vagner,
V. Vagnoni,
A. Valassi,
S. Valat,
G. Valenti,
H. Van Hecke,
C.B. Van Hulse,
R. Vazquez Gomez,
P. Vazquez Regueiro,
S. Vecchi,
M. van Veghel,
J.J. Velthuis,
M. Veltri,
A. Venkateswaran,
M. Vernet,
M. Veronesi,
M. Vesterinen,
J.V. Viana Barbosa,
D.  Vieira,
M. Vieites Diaz,
H. Viemann,
X. Vilasis-Cardona,
A. Vitkovskiy,
V. Volkov,
A. Vollhardt,
D. Vom Bruch,
B. Voneki,
A. Vorobyev,
V. Vorobyev,
N. Voropaev,
J.A. de Vries,
C. V{\'a}zquez Sierra,
R. Waldi,
J. Walsh,
J. Wang,
J. Wang,
M. Wang,
Y. Wang,
Z. Wang,
D.R. Ward,
H.M. Wark,
N.K. Watson,
D. Websdale,
A. Weiden,
C. Weisser,
B.D.C. Westhenry,
D.J. White,
M. Whitehead,
D. Wiedner,
G. Wilkinson,
M. Wilkinson,
I. Williams,
M.R.J. Williams,
M. Williams,
T. Williams,
F.F. Wilson,
M. Winn,
W. Wislicki,
M. Witek,
G. Wormser,
S.A. Wotton,
H. Wu,
K. Wyllie,
Z. Xiang,
D. Xiao,
Y. Xie,
H. Xing,
A. Xu,
L. Xu,
M. Xu,
Q. Xu,
Z. Xu,
Z. Xu,
Z. Yang,
Z. Yang,
Y. Yao,
L.E. Yeomans,
H. Yin,
J. Yu,
X. Yuan,
O. Yushchenko,
K.A. Zarebski,
M. Zavertyaev,
M. Zdybal,
M. Zeng,
D. Zhang,
L. Zhang,
S. Zhang,
W.C. Zhang,
Y. Zhang,
A. Zhelezov,
Y. Zheng,
X. Zhou,
Y. Zhou,
V. Zhovkovska,
X. Zhu,
V. Zhukov,
J.B. Zonneveld,
S. Zucchelli


==> Makefile <==
# $Id: Makefile 87305 2016-02-08 13:50:32Z lafferty $
# ===============================================================================
# Purpose: simple Makefile to streamline processing latex document (just say "make" to execute)
# Author: Tomasz Skwarnicki
# Created on: 2010-09-24
# A few changes by Patrick Koppenburg on 2015-06-26
# ===============================================================================

# name of the main latex file (do not include .tex)
MAIN = main

# name of the target - change that to something descriptive, like paper-v0, Bs2PhiPhi-ANA-v1, etc...
TARGET = template

# name of command to perform Latex (either pdflatex or latex)
LATEX = pdflatex

ifeq ($(LATEX),pdflatex)
	FIGEXT = .pdf
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN)
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl
	MAKEMAINCOUNT= sed 's\#{wordcount}{false}\#{wordcount}{true}\#' main-prl.tex > main-count.tex
	BUILDCOMMANDCOUNT= $(MAKEMAINCOUNT) && rm -f $(MAIN)-count.aux && $(LATEX) $(MAIN)-count && bibtex $(MAIN)-count >/dev/null; true && $(LATEX) $(MAIN)-count && ./wordcount.sh $(MAIN)-count && rm wordcount.pdf main-count* 
else
	FIGEXT = .eps
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN) && dvips -z -o $(MAIN).ps $(MAIN) && ps2pdf $(MAIN).ps && rm -f head.tmp body.tmp
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl && dvips -z -o $(MAIN)-prl.ps $(MAIN)-prl && ps2pdf $(MAIN)-prl.ps && rm -f head.tmp body.tmp
	BUILDCOMMANDCOUNT=
endif

# list of all source files
TEXSOURCES = $(wildcard *.tex) $(wildcard *.bib) $(wildcard *.bst)
FIGSOURCES = $(wildcard figs/*$(FIGEXT))
SOURCES    = $(TEXSOURCES) $(FIGSOURCES)

# define output (could be making .ps instead)
OUTPUT = $(TARGET)$(MAINEXT)

# cp temporary main.pdf to target.
$(OUTPUT): $(MAIN)$(MAINEXT)
	cp $(MAIN)$(MAINEXT) $(OUTPUT)

# prescription how to make output (your favorite commands to process latex)
# do latex twice to make sure that all cross-references are updated 
$(MAIN)$(MAINEXT): $(SOURCES) Makefile
	$(BUILDCOMMAND)

# just so we can say "make all" without knowing the output name
all: $(OUTPUT)

# remove temporary files (good idea to say "make clean" before putting things back into repository)
.PHONY : clean
clean:
	rm -f *~ *.aux *.log *.bbl *.blg *.dvi *.tmp *.out *.blg *.bbl $(OUTPUT) $(MAIN)$(MAINEXT) $(MAIN).ps $(MAIN)-prl.ps $(MAIN)-prlNotes.bib

# remove output file
rmout: 
	rm $(OUTPUT) $(MAIN)$(MAINEXT)

# Make the PRL version
prl: 
	$(BUILDCOMMANDPRL)

# Make the PRL version
count: 
	$(BUILDCOMMANDCOUNT)
	@echo ''
	@echo 'Figures:   Add 20+150/(aspect ratio) per figure'
	@echo 'Equations: Add 16 words per row (single column) '
	@echo 'Tables:    Add 13 words plus 6.5 words per line (single column)'
	@echo 


==> lhcb-symbols-list.tex <==
% This is an automatically generated appendix to template.tex. 
% When included it will show all the symbols defined in lhcb-symbols-def.tex.
%
% To regenerate with the latest definitions run the script python listsymbols.py

\section{List of all symbols}
\label{sec:listofsymbols}
\subsection{Experiments}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash lhcb} & \lhcb & \texttt{\textbackslash atlas} & \atlas & \texttt{\textbackslash cms} & \cms \\
\texttt{\textbackslash alice} & \alice & \texttt{\textbackslash babar} & \babar & \texttt{\textbackslash belle} & \belle \\
\texttt{\textbackslash belletwo} & \belletwo & \texttt{\textbackslash besiii} & \besiii & \texttt{\textbackslash cleo} & \cleo \\
\texttt{\textbackslash cdf} & \cdf & \texttt{\textbackslash dzero} & \dzero & \texttt{\textbackslash aleph} & \aleph \\
\texttt{\textbackslash delphi} & \delphi & \texttt{\textbackslash opal} & \opal & \texttt{\textbackslash lthree} & \lthree \\
\texttt{\textbackslash sld} & \sld & \texttt{\textbackslash cern} & \cern & \texttt{\textbackslash lhc} & \lhc \\
\texttt{\textbackslash lep} & \lep & \texttt{\textbackslash tevatron} & \tevatron & \texttt{\textbackslash bfactories} & \bfactories \\
\texttt{\textbackslash bfactory} & \bfactory & \texttt{\textbackslash upgradeone} & \upgradeone & \texttt{\textbackslash upgradetwo} & \upgradetwo \\
\end{tabular*}

\subsubsection{LHCb sub-detectors and sub-systems}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash velo} & \velo & \texttt{\textbackslash rich} & \rich & \texttt{\textbackslash richone} & \richone \\
\texttt{\textbackslash richtwo} & \richtwo & \texttt{\textbackslash ttracker} & \ttracker & \texttt{\textbackslash intr} & \intr \\
\texttt{\textbackslash st} & \st & \texttt{\textbackslash ot} & \ot & \texttt{\textbackslash herschel} & \herschel \\
\texttt{\textbackslash spd} & \spd & \texttt{\textbackslash presh} & \presh & \texttt{\textbackslash ecal} & \ecal \\
\texttt{\textbackslash hcal} & \hcal & \texttt{\textbackslash MagUp} & \MagUp & \texttt{\textbackslash MagDown} & \MagDown \\
\texttt{\textbackslash ode} & \ode & \texttt{\textbackslash daq} & \daq & \texttt{\textbackslash tfc} & \tfc \\
\texttt{\textbackslash ecs} & \ecs & \texttt{\textbackslash lone} & \lone & \texttt{\textbackslash hlt} & \hlt \\
\texttt{\textbackslash hltone} & \hltone & \texttt{\textbackslash hlttwo} & \hlttwo &  \\
\end{tabular*}

\subsection{Particles}
\subsubsection{Leptons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash electron} & \electron & \texttt{\textbackslash en} & \en & \texttt{\textbackslash ep} & \ep \\
\texttt{\textbackslash epm} & \epm & \texttt{\textbackslash emp} & \emp & \texttt{\textbackslash epem} & \epem \\
\texttt{\textbackslash muon} & \muon & \texttt{\textbackslash mup} & \mup & \texttt{\textbackslash mun} & \mun \\
\texttt{\textbackslash mupm} & \mupm & \texttt{\textbackslash mump} & \mump & \texttt{\textbackslash mumu} & \mumu \\
\texttt{\textbackslash tauon} & \tauon & \texttt{\textbackslash taup} & \taup & \texttt{\textbackslash taum} & \taum \\
\texttt{\textbackslash taupm} & \taupm & \texttt{\textbackslash taump} & \taump & \texttt{\textbackslash tautau} & \tautau \\
\texttt{\textbackslash lepton} & \lepton & \texttt{\textbackslash ellm} & \ellm & \texttt{\textbackslash ellp} & \ellp \\
\texttt{\textbackslash ellell} & \ellell & \texttt{\textbackslash neu} & \neu & \texttt{\textbackslash neub} & \neub \\
\texttt{\textbackslash neue} & \neue & \texttt{\textbackslash neueb} & \neueb & \texttt{\textbackslash neum} & \neum \\
\texttt{\textbackslash neumb} & \neumb & \texttt{\textbackslash neut} & \neut & \texttt{\textbackslash neutb} & \neutb \\
\texttt{\textbackslash neul} & \neul & \texttt{\textbackslash neulb} & \neulb &  \\
\end{tabular*}

\subsubsection{Gauge bosons and scalars}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash g} & \g & \texttt{\textbackslash H} & \H & \texttt{\textbackslash Hp} & \Hp \\
\texttt{\textbackslash Hm} & \Hm & \texttt{\textbackslash Hpm} & \Hpm & \texttt{\textbackslash W} & \W \\
\texttt{\textbackslash Wp} & \Wp & \texttt{\textbackslash Wm} & \Wm & \texttt{\textbackslash Wpm} & \Wpm \\
\texttt{\textbackslash Z} & \Z &  \\
\end{tabular*}

\subsubsection{Quarks}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash quark} & \quark & \texttt{\textbackslash quarkbar} & \quarkbar & \texttt{\textbackslash qqbar} & \qqbar \\
\texttt{\textbackslash uquark} & \uquark & \texttt{\textbackslash uquarkbar} & \uquarkbar & \texttt{\textbackslash uubar} & \uubar \\
\texttt{\textbackslash dquark} & \dquark & \texttt{\textbackslash dquarkbar} & \dquarkbar & \texttt{\textbackslash ddbar} & \ddbar \\
\texttt{\textbackslash squark} & \squark & \texttt{\textbackslash squarkbar} & \squarkbar & \texttt{\textbackslash ssbar} & \ssbar \\
\texttt{\textbackslash cquark} & \cquark & \texttt{\textbackslash cquarkbar} & \cquarkbar & \texttt{\textbackslash ccbar} & \ccbar \\
\texttt{\textbackslash bquark} & \bquark & \texttt{\textbackslash bquarkbar} & \bquarkbar & \texttt{\textbackslash bbbar} & \bbbar \\
\texttt{\textbackslash tquark} & \tquark & \texttt{\textbackslash tquarkbar} & \tquarkbar & \texttt{\textbackslash ttbar} & \ttbar \\
\end{tabular*}

\subsubsection{Light mesons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash hadron} & \hadron & \texttt{\textbackslash pion} & \pion & \texttt{\textbackslash piz} & \piz \\
\texttt{\textbackslash pip} & \pip & \texttt{\textbackslash pim} & \pim & \texttt{\textbackslash pipm} & \pipm \\
\texttt{\textbackslash pimp} & \pimp & \texttt{\textbackslash rhomeson} & \rhomeson & \texttt{\textbackslash rhoz} & \rhoz \\
\texttt{\textbackslash rhop} & \rhop & \texttt{\textbackslash rhom} & \rhom & \texttt{\textbackslash rhopm} & \rhopm \\
\texttt{\textbackslash rhomp} & \rhomp & \texttt{\textbackslash kaon} & \kaon & \texttt{\textbackslash Kbar} & \Kbar \\
\texttt{\textbackslash Kb} & \Kb & \texttt{\textbackslash KorKbar} & \KorKbar & \texttt{\textbackslash Kz} & \Kz \\
\texttt{\textbackslash Kzb} & \Kzb & \texttt{\textbackslash Kp} & \Kp & \texttt{\textbackslash Km} & \Km \\
\texttt{\textbackslash Kpm} & \Kpm & \texttt{\textbackslash Kmp} & \Kmp & \texttt{\textbackslash KS} & \KS \\
\texttt{\textbackslash Vzero} & \Vzero & \texttt{\textbackslash KL} & \KL & \texttt{\textbackslash Kstarz} & \Kstarz \\
\texttt{\textbackslash Kstarzb} & \Kstarzb & \texttt{\textbackslash Kstar} & \Kstar & \texttt{\textbackslash Kstarb} & \Kstarb \\
\texttt{\textbackslash Kstarp} & \Kstarp & \texttt{\textbackslash Kstarm} & \Kstarm & \texttt{\textbackslash Kstarpm} & \Kstarpm \\
\texttt{\textbackslash Kstarmp} & \Kstarmp & \texttt{\textbackslash KorKbarz} & \KorKbarz & \texttt{\textbackslash etaz} & \etaz \\
\texttt{\textbackslash etapr} & \etapr & \texttt{\textbackslash phiz} & \phiz & \texttt{\textbackslash omegaz} & \omegaz \\
\end{tabular*}

\subsubsection{Charmed mesons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Dbar} & \Dbar & \texttt{\textbackslash D} & \D & \texttt{\textbackslash Db} & \Db \\
\texttt{\textbackslash DorDbar} & \DorDbar & \texttt{\textbackslash Dz} & \Dz & \texttt{\textbackslash Dzb} & \Dzb \\
\texttt{\textbackslash Dp} & \Dp & \texttt{\textbackslash Dm} & \Dm & \texttt{\textbackslash Dpm} & \Dpm \\
\texttt{\textbackslash Dmp} & \Dmp & \texttt{\textbackslash Dstar} & \Dstar & \texttt{\textbackslash Dstarb} & \Dstarb \\
\texttt{\textbackslash Dstarz} & \Dstarz & \texttt{\textbackslash Dstarzb} & \Dstarzb & \texttt{\textbackslash theDstarz} & \theDstarz \\
\texttt{\textbackslash theDstarzb} & \theDstarzb & \texttt{\textbackslash Dstarp} & \Dstarp & \texttt{\textbackslash Dstarm} & \Dstarm \\
\texttt{\textbackslash Dstarpm} & \Dstarpm & \texttt{\textbackslash Dstarmp} & \Dstarmp & \texttt{\textbackslash theDstarp} & \theDstarp \\
\texttt{\textbackslash theDstarm} & \theDstarm & \texttt{\textbackslash theDstarpm} & \theDstarpm & \texttt{\textbackslash theDstarmp} & \theDstarmp \\
\texttt{\textbackslash Ds} & \Ds & \texttt{\textbackslash Dsp} & \Dsp & \texttt{\textbackslash Dsm} & \Dsm \\
\texttt{\textbackslash Dspm} & \Dspm & \texttt{\textbackslash Dsmp} & \Dsmp & \texttt{\textbackslash Dss} & \Dss \\
\texttt{\textbackslash Dssp} & \Dssp & \texttt{\textbackslash Dssm} & \Dssm & \texttt{\textbackslash Dsspm} & \Dsspm \\
\texttt{\textbackslash Dssmp} & \Dssmp &  \\
\end{tabular*}

\subsubsection{Beauty mesons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash B} & \B & \texttt{\textbackslash Bbar} & \Bbar & \texttt{\textbackslash Bb} & \Bb \\
\texttt{\textbackslash BorBbar} & \BorBbar & \texttt{\textbackslash Bz} & \Bz & \texttt{\textbackslash Bzb} & \Bzb \\
\texttt{\textbackslash Bd} & \Bd & \texttt{\textbackslash Bdb} & \Bdb & \texttt{\textbackslash BdorBdbar} & \BdorBdbar \\
\texttt{\textbackslash Bu} & \Bu & \texttt{\textbackslash Bub} & \Bub & \texttt{\textbackslash Bp} & \Bp \\
\texttt{\textbackslash Bm} & \Bm & \texttt{\textbackslash Bpm} & \Bpm & \texttt{\textbackslash Bmp} & \Bmp \\
\texttt{\textbackslash Bs} & \Bs & \texttt{\textbackslash Bsb} & \Bsb & \texttt{\textbackslash BsorBsbar} & \BsorBsbar \\
\texttt{\textbackslash Bc} & \Bc & \texttt{\textbackslash Bcp} & \Bcp & \texttt{\textbackslash Bcm} & \Bcm \\
\texttt{\textbackslash Bcpm} & \Bcpm & \texttt{\textbackslash Bds} & \Bds & \texttt{\textbackslash Bdsb} & \Bdsb \\
\texttt{\textbackslash BdorBs} & \BdorBs &  \\
\end{tabular*}

\subsubsection{Onia}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash jpsi} & \jpsi & \texttt{\textbackslash psitwos} & \psitwos & \texttt{\textbackslash psiprpr} & \psiprpr \\
\texttt{\textbackslash etac} & \etac & \texttt{\textbackslash chic} & \chic & \texttt{\textbackslash chiczero} & \chiczero \\
\texttt{\textbackslash chicone} & \chicone & \texttt{\textbackslash chictwo} & \chictwo & \texttt{\textbackslash chicJ} & \chicJ \\
\texttt{\textbackslash Upsilonres} & \Upsilonres & \texttt{\textbackslash OneS} & \OneS & \texttt{\textbackslash TwoS} & \TwoS \\
\texttt{\textbackslash ThreeS} & \ThreeS & \texttt{\textbackslash FourS} & \FourS & \texttt{\textbackslash FiveS} & \FiveS \\
\texttt{\textbackslash chib} & \chib & \texttt{\textbackslash chibzero} & \chibzero & \texttt{\textbackslash chibone} & \chibone \\
\texttt{\textbackslash chibtwo} & \chibtwo & \texttt{\textbackslash chibJ} & \chibJ &  \\
\end{tabular*}

\subsubsection{Light Baryons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash proton} & \proton & \texttt{\textbackslash antiproton} & \antiproton & \texttt{\textbackslash neutron} & \neutron \\
\texttt{\textbackslash antineutron} & \antineutron & \texttt{\textbackslash Deltares} & \Deltares & \texttt{\textbackslash Deltaresbar} & \Deltaresbar \\
\texttt{\textbackslash Lz} & \Lz & \texttt{\textbackslash Lbar} & \Lbar & \texttt{\textbackslash LorLbar} & \LorLbar \\
\texttt{\textbackslash Lambdares} & \Lambdares & \texttt{\textbackslash Lambdaresbar} & \Lambdaresbar & \texttt{\textbackslash Sigmares} & \Sigmares \\
\texttt{\textbackslash Sigmaz} & \Sigmaz & \texttt{\textbackslash Sigmap} & \Sigmap & \texttt{\textbackslash Sigmam} & \Sigmam \\
\texttt{\textbackslash Sigmaresbar} & \Sigmaresbar & \texttt{\textbackslash Sigmabarz} & \Sigmabarz & \texttt{\textbackslash Sigmabarp} & \Sigmabarp \\
\texttt{\textbackslash Sigmabarm} & \Sigmabarm & \texttt{\textbackslash Xires} & \Xires & \texttt{\textbackslash Xiresz} & \Xiresz \\
\texttt{\textbackslash Xiresm} & \Xiresm & \texttt{\textbackslash Xiresbar} & \Xiresbar & \texttt{\textbackslash Xiresbarz} & \Xiresbarz \\
\texttt{\textbackslash Xiresbarp} & \Xiresbarp & \texttt{\textbackslash Omegares} & \Omegares & \texttt{\textbackslash Omegaresbar} & \Omegaresbar \\
\texttt{\textbackslash Omegam} & \Omegam & \texttt{\textbackslash Omegabarp} & \Omegabarp &  \\
\end{tabular*}

\subsubsection{Charmed Baryons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Lc} & \Lc & \texttt{\textbackslash Lcbar} & \Lcbar & \texttt{\textbackslash Xic} & \Xic \\
\texttt{\textbackslash Xicz} & \Xicz & \texttt{\textbackslash Xicp} & \Xicp & \texttt{\textbackslash Xicbar} & \Xicbar \\
\texttt{\textbackslash Xicbarz} & \Xicbarz & \texttt{\textbackslash Xicbarm} & \Xicbarm & \texttt{\textbackslash Omegac} & \Omegac \\
\texttt{\textbackslash Omegacbar} & \Omegacbar & \texttt{\textbackslash Xicc} & \Xicc & \texttt{\textbackslash Xiccbar} & \Xiccbar \\
\texttt{\textbackslash Xiccp} & \Xiccp & \texttt{\textbackslash Xiccpp} & \Xiccpp & \texttt{\textbackslash Xiccbarm} & \Xiccbarm \\
\texttt{\textbackslash Xiccbarmm} & \Xiccbarmm & \texttt{\textbackslash Omegacc} & \Omegacc & \texttt{\textbackslash Omegaccbar} & \Omegaccbar \\
\texttt{\textbackslash Omegaccc} & \Omegaccc & \texttt{\textbackslash Omegacccbar} & \Omegacccbar &  \\
\end{tabular*}

\subsubsection{Beauty Baryons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Lb} & \Lb & \texttt{\textbackslash Lbbar} & \Lbbar & \texttt{\textbackslash Sigmab} & \Sigmab \\
\texttt{\textbackslash Sigmabp} & \Sigmabp & \texttt{\textbackslash Sigmabz} & \Sigmabz & \texttt{\textbackslash Sigmabm} & \Sigmabm \\
\texttt{\textbackslash Sigmabpm} & \Sigmabpm & \texttt{\textbackslash Sigmabbar} & \Sigmabbar & \texttt{\textbackslash Sigmabbarp} & \Sigmabbarp \\
\texttt{\textbackslash Sigmabbarz} & \Sigmabbarz & \texttt{\textbackslash Sigmabbarm} & \Sigmabbarm & \texttt{\textbackslash Sigmabbarpm} & \Sigmabbarpm \\
\texttt{\textbackslash Xib} & \Xib & \texttt{\textbackslash Xibz} & \Xibz & \texttt{\textbackslash Xibm} & \Xibm \\
\texttt{\textbackslash Xibbar} & \Xibbar & \texttt{\textbackslash Xibbarz} & \Xibbarz & \texttt{\textbackslash Xibbarp} & \Xibbarp \\
\texttt{\textbackslash Omegab} & \Omegab & \texttt{\textbackslash Omegabbar} & \Omegabbar &  \\
\end{tabular*}

\subsection{Physics symbols}
\subsubsection{Decays}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BF} & \BF & \texttt{\textbackslash BR} & \BR & \texttt{\textbackslash BRvis} & \BRvis \\
\texttt{\textbackslash ra} & \ra & \texttt{\textbackslash to} & \to &  \\
\end{tabular*}

\subsubsection{Lifetimes}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tauBs} & \tauBs & \texttt{\textbackslash tauBd} & \tauBd & \texttt{\textbackslash tauBz} & \tauBz \\
\texttt{\textbackslash tauBu} & \tauBu & \texttt{\textbackslash tauDp} & \tauDp & \texttt{\textbackslash tauDz} & \tauDz \\
\texttt{\textbackslash tauL} & \tauL & \texttt{\textbackslash tauH} & \tauH &  \\
\end{tabular*}

\subsubsection{Masses}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash mBd} & \mBd & \texttt{\textbackslash mBp} & \mBp & \texttt{\textbackslash mBs} & \mBs \\
\texttt{\textbackslash mBc} & \mBc & \texttt{\textbackslash mLb} & \mLb &  \\
\end{tabular*}

\subsubsection{EW theory, groups}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash grpsuthree} & \grpsuthree & \texttt{\textbackslash grpsutw} & \grpsutw & \texttt{\textbackslash grpuone} & \grpuone \\
\texttt{\textbackslash ssqtw} & \ssqtw & \texttt{\textbackslash csqtw} & \csqtw & \texttt{\textbackslash stw} & \stw \\
\texttt{\textbackslash ctw} & \ctw & \texttt{\textbackslash ssqtwef} & \ssqtwef & \texttt{\textbackslash csqtwef} & \csqtwef \\
\texttt{\textbackslash stwef} & \stwef & \texttt{\textbackslash ctwef} & \ctwef & \texttt{\textbackslash gv} & \gv \\
\texttt{\textbackslash ga} & \ga & \texttt{\textbackslash order} & \order & \texttt{\textbackslash ordalph} & \ordalph \\
\texttt{\textbackslash ordalsq} & \ordalsq & \texttt{\textbackslash ordalcb} & \ordalcb &  \\
\end{tabular*}

\subsubsection{QCD parameters}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash as} & \as & \texttt{\textbackslash MSb} & \MSb & \texttt{\textbackslash lqcd} & \lqcd \\
\texttt{\textbackslash qsq} & \qsq &  \\
\end{tabular*}

\subsubsection{CKM, \boldmath \CP violation}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash eps} & \eps & \texttt{\textbackslash epsK} & \epsK & \texttt{\textbackslash epsB} & \epsB \\
\texttt{\textbackslash epsp} & \epsp & \texttt{\textbackslash CP} & \CP & \texttt{\textbackslash CPT} & \CPT \\
\texttt{\textbackslash T} & \T & \texttt{\textbackslash rhobar} & \rhobar & \texttt{\textbackslash etabar} & \etabar \\
\texttt{\textbackslash Vud} & \Vud & \texttt{\textbackslash Vcd} & \Vcd & \texttt{\textbackslash Vtd} & \Vtd \\
\texttt{\textbackslash Vus} & \Vus & \texttt{\textbackslash Vcs} & \Vcs & \texttt{\textbackslash Vts} & \Vts \\
\texttt{\textbackslash Vub} & \Vub & \texttt{\textbackslash Vcb} & \Vcb & \texttt{\textbackslash Vtb} & \Vtb \\
\texttt{\textbackslash Vuds} & \Vuds & \texttt{\textbackslash Vcds} & \Vcds & \texttt{\textbackslash Vtds} & \Vtds \\
\texttt{\textbackslash Vuss} & \Vuss & \texttt{\textbackslash Vcss} & \Vcss & \texttt{\textbackslash Vtss} & \Vtss \\
\texttt{\textbackslash Vubs} & \Vubs & \texttt{\textbackslash Vcbs} & \Vcbs & \texttt{\textbackslash Vtbs} & \Vtbs \\
\end{tabular*}

\subsubsection{Oscillations}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash dm} & \dm & \texttt{\textbackslash dms} & \dms & \texttt{\textbackslash dmd} & \dmd \\
\texttt{\textbackslash DG} & \DG & \texttt{\textbackslash DGs} & \DGs & \texttt{\textbackslash DGd} & \DGd \\
\texttt{\textbackslash Gs} & \Gs & \texttt{\textbackslash Gd} & \Gd & \texttt{\textbackslash MBq} & \MBq \\
\texttt{\textbackslash DGq} & \DGq & \texttt{\textbackslash Gq} & \Gq & \texttt{\textbackslash dmq} & \dmq \\
\texttt{\textbackslash GL} & \GL & \texttt{\textbackslash GH} & \GH & \texttt{\textbackslash DGsGs} & \DGsGs \\
\texttt{\textbackslash Delm} & \Delm & \texttt{\textbackslash ACP} & \ACP & \texttt{\textbackslash Adir} & \Adir \\
\texttt{\textbackslash Amix} & \Amix & \texttt{\textbackslash ADelta} & \ADelta & \texttt{\textbackslash phid} & \phid \\
\texttt{\textbackslash sinphid} & \sinphid & \texttt{\textbackslash phis} & \phis & \texttt{\textbackslash betas} & \betas \\
\texttt{\textbackslash sbetas} & \sbetas & \texttt{\textbackslash stbetas} & \stbetas & \texttt{\textbackslash stphis} & \stphis \\
\texttt{\textbackslash sinphis} & \sinphis &  \\
\end{tabular*}

\subsubsection{Tagging}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash edet} & \edet & \texttt{\textbackslash erec} & \erec & \texttt{\textbackslash esel} & \esel \\
\texttt{\textbackslash etrg} & \etrg & \texttt{\textbackslash etot} & \etot & \texttt{\textbackslash mistag} & \mistag \\
\texttt{\textbackslash wcomb} & \wcomb & \texttt{\textbackslash etag} & \etag & \texttt{\textbackslash etagcomb} & \etagcomb \\
\texttt{\textbackslash effeff} & \effeff & \texttt{\textbackslash effeffcomb} & \effeffcomb & \texttt{\textbackslash efftag} & \efftag \\
\texttt{\textbackslash effD} & \effD & \texttt{\textbackslash etagprompt} & \etagprompt & \texttt{\textbackslash etagLL} & \etagLL \\
\end{tabular*}

\subsubsection{Key decay channels}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BdToKstmm} & \BdToKstmm & \texttt{\textbackslash BdbToKstmm} & \BdbToKstmm & \texttt{\textbackslash BsToJPsiPhi} & \BsToJPsiPhi \\
\texttt{\textbackslash BdToJPsiKst} & \BdToJPsiKst & \texttt{\textbackslash BdbToJPsiKst} & \BdbToJPsiKst & \texttt{\textbackslash BsPhiGam} & \BsPhiGam \\
\texttt{\textbackslash BdKstGam} & \BdKstGam & \texttt{\textbackslash BTohh} & \BTohh & \texttt{\textbackslash BdTopipi} & \BdTopipi \\
\texttt{\textbackslash BdToKpi} & \BdToKpi & \texttt{\textbackslash BsToKK} & \BsToKK & \texttt{\textbackslash BsTopiK} & \BsTopiK \\
\texttt{\textbackslash Cpipi} & \Cpipi & \texttt{\textbackslash Spipi} & \Spipi & \texttt{\textbackslash CKK} & \CKK \\
\texttt{\textbackslash SKK} & \SKK & \texttt{\textbackslash ADGKK} & \ADGKK &  \\
\end{tabular*}

\subsubsection{Rare decays}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BdKstee} & \BdKstee & \texttt{\textbackslash BdbKstee} & \BdbKstee & \texttt{\textbackslash bsll} & \bsll \\
\texttt{\textbackslash AFB} & \AFB & \texttt{\textbackslash FL} & \FL & \texttt{\textbackslash AT\#1 \textbackslash AT2} & \AT2 \\
\texttt{\textbackslash btosgam} & \btosgam & \texttt{\textbackslash btodgam} & \btodgam & \texttt{\textbackslash Bsmm} & \Bsmm \\
\texttt{\textbackslash Bdmm} & \Bdmm & \texttt{\textbackslash Bsee} & \Bsee & \texttt{\textbackslash Bdee} & \Bdee \\
\texttt{\textbackslash ctl} & \ctl & \texttt{\textbackslash ctk} & \ctk &  \\
\end{tabular*}

\subsubsection{Wilson coefficients and operators}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash C\#1 \textbackslash C9} & \C9 & \texttt{\textbackslash Cp\#1 \textbackslash Cp7} & \Cp7 & \texttt{\textbackslash Ceff\#1 \textbackslash Ceff9  } & \Ceff9   \\
\texttt{\textbackslash Cpeff\#1 \textbackslash Cpeff7} & \Cpeff7 & \texttt{\textbackslash Ope\#1 \textbackslash Ope2} & \Ope2 & \texttt{\textbackslash Opep\#1 \textbackslash Opep7} & \Opep7 \\
\end{tabular*}

\subsubsection{Charm}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash xprime} & \xprime & \texttt{\textbackslash yprime} & \yprime & \texttt{\textbackslash ycp} & \ycp \\
\texttt{\textbackslash agamma} & \agamma & \texttt{\textbackslash dkpicf} & \dkpicf &  \\
\end{tabular*}

\subsubsection{QM}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash bra[1] \textbackslash bra\{a\}} & \bra{a} & \texttt{\textbackslash ket[1] \textbackslash ket\{b\}} & \ket{b} & \texttt{\textbackslash braket[2] \textbackslash braket\{a\}\{b\}} & \braket{a}{b} \\
\end{tabular*}

\subsection{Units (these macros add a small space in front)}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash unit[1] \textbackslash unit\{kg\}   } & \unit{kg}    &  \\
\end{tabular*}

\subsubsection{Energy and momentum }
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tev} & \tev & \texttt{\textbackslash gev} & \gev & \texttt{\textbackslash mev} & \mev \\
\texttt{\textbackslash kev} & \kev & \texttt{\textbackslash ev} & \ev & \texttt{\textbackslash mevc} & \mevc \\
\texttt{\textbackslash gevc} & \gevc & \texttt{\textbackslash mevcc} & \mevcc & \texttt{\textbackslash gevcc} & \gevcc \\
\texttt{\textbackslash gevgevcc} & \gevgevcc & \texttt{\textbackslash gevgevcccc} & \gevgevcccc &  \\
\end{tabular*}

\subsubsection{Distance and area (these macros add a small space)}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash km} & \km & \texttt{\textbackslash m} & \m & \texttt{\textbackslash ma} & \ma \\
\texttt{\textbackslash cm} & \cm & \texttt{\textbackslash cma} & \cma & \texttt{\textbackslash mm} & \mm \\
\texttt{\textbackslash mma} & \mma & \texttt{\textbackslash mum} & \mum & \texttt{\textbackslash muma} & \muma \\
\texttt{\textbackslash nm} & \nm & \texttt{\textbackslash fm} & \fm & \texttt{\textbackslash barn} & \barn \\
\texttt{\textbackslash mbarn} & \mbarn & \texttt{\textbackslash mub} & \mub & \texttt{\textbackslash nb} & \nb \\
\texttt{\textbackslash invnb} & \invnb & \texttt{\textbackslash pb} & \pb & \texttt{\textbackslash invpb} & \invpb \\
\texttt{\textbackslash fb} & \fb & \texttt{\textbackslash invfb} & \invfb & \texttt{\textbackslash ab} & \ab \\
\texttt{\textbackslash invab} & \invab &  \\
\end{tabular*}

\subsubsection{Time }
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash sec} & \sec & \texttt{\textbackslash ms} & \ms & \texttt{\textbackslash mus} & \mus \\
\texttt{\textbackslash ns} & \ns & \texttt{\textbackslash ps} & \ps & \texttt{\textbackslash fs} & \fs \\
\texttt{\textbackslash mhz} & \mhz & \texttt{\textbackslash khz} & \khz & \texttt{\textbackslash hz} & \hz \\
\texttt{\textbackslash invps} & \invps & \texttt{\textbackslash invns} & \invns & \texttt{\textbackslash yr} & \yr \\
\texttt{\textbackslash hr} & \hr &  \\
\end{tabular*}

\subsubsection{Temperature}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash degc} & \degc & \texttt{\textbackslash degk} & \degk &  \\
\end{tabular*}

\subsubsection{Material lengths, radiation}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Xrad} & \Xrad & \texttt{\textbackslash NIL} & \NIL & \texttt{\textbackslash mip} & \mip \\
\texttt{\textbackslash neutroneq} & \neutroneq & \texttt{\textbackslash neqcmcm} & \neqcmcm & \texttt{\textbackslash kRad} & \kRad \\
\texttt{\textbackslash MRad} & \MRad & \texttt{\textbackslash ci} & \ci & \texttt{\textbackslash mci} & \mci \\
\end{tabular*}

\subsubsection{Uncertainties}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash sx} & \sx & \texttt{\textbackslash sy} & \sy & \texttt{\textbackslash sz} & \sz \\
\texttt{\textbackslash stat} & \stat & \texttt{\textbackslash syst} & \syst &  \\
\end{tabular*}

\subsubsection{Maths}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash order} & \order & \texttt{\textbackslash chisq} & \chisq & \texttt{\textbackslash chisqndf} & \chisqndf \\
\texttt{\textbackslash chisqip} & \chisqip & \texttt{\textbackslash chisqvs} & \chisqvs & \texttt{\textbackslash chisqvtx} & \chisqvtx \\
\texttt{\textbackslash chisqvtxndf} & \chisqvtxndf & \texttt{\textbackslash deriv} & \deriv & \texttt{\textbackslash gsim} & \gsim \\
\texttt{\textbackslash lsim} & \lsim & \texttt{\textbackslash mean[1] \textbackslash mean\{x\}} & \mean{x} & \texttt{\textbackslash abs[1] \textbackslash abs\{x\}} & \abs{x} \\
\texttt{\textbackslash Real} & \Real & \texttt{\textbackslash Imag} & \Imag & \texttt{\textbackslash PDF} & \PDF \\
\texttt{\textbackslash sPlot} & \sPlot & \texttt{\textbackslash sFit} & \sFit &  \\
\end{tabular*}

\subsection{Kinematics}
\subsubsection{Energy, Momenta}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Ebeam} & \Ebeam & \texttt{\textbackslash sqs} & \sqs & \texttt{\textbackslash sqsnn} & \sqsnn \\
\texttt{\textbackslash pt} & \pt & \texttt{\textbackslash ptsq} & \ptsq & \texttt{\textbackslash ptot} & \ptot \\
\texttt{\textbackslash et} & \et & \texttt{\textbackslash mt} & \mt & \texttt{\textbackslash dpp} & \dpp \\
\texttt{\textbackslash msq} & \msq & \texttt{\textbackslash dedx} & \dedx &  \\
\end{tabular*}

\subsubsection{PID}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash dllkpi} & \dllkpi & \texttt{\textbackslash dllppi} & \dllppi & \texttt{\textbackslash dllepi} & \dllepi \\
\texttt{\textbackslash dllmupi} & \dllmupi &  \\
\end{tabular*}

\subsubsection{Geometry}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash degrees} & \degrees & \texttt{\textbackslash krad} & \krad & \texttt{\textbackslash mrad} & \mrad \\
\texttt{\textbackslash rad} & \rad &  \\
\end{tabular*}

\subsubsection{Accelerator}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash betastar} & \betastar & \texttt{\textbackslash lum} & \lum & \texttt{\textbackslash intlum[1] \textbackslash intlum\{2 \,\invfb\}} & \intlum{2 \,\invfb} \\
\end{tabular*}

\subsection{Software}
\subsubsection{Programs}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash bcvegpy} & \bcvegpy & \texttt{\textbackslash boole} & \boole & \texttt{\textbackslash brunel} & \brunel \\
\texttt{\textbackslash davinci} & \davinci & \texttt{\textbackslash dirac} & \dirac & \texttt{\textbackslash evtgen} & \evtgen \\
\texttt{\textbackslash fewz} & \fewz & \texttt{\textbackslash fluka} & \fluka & \texttt{\textbackslash ganga} & \ganga \\
\texttt{\textbackslash gaudi} & \gaudi & \texttt{\textbackslash gauss} & \gauss & \texttt{\textbackslash geant} & \geant \\
\texttt{\textbackslash hepmc} & \hepmc & \texttt{\textbackslash herwig} & \herwig & \texttt{\textbackslash moore} & \moore \\
\texttt{\textbackslash neurobayes} & \neurobayes & \texttt{\textbackslash photos} & \photos & \texttt{\textbackslash powheg} & \powheg \\
\texttt{\textbackslash pythia} & \pythia & \texttt{\textbackslash resbos} & \resbos & \texttt{\textbackslash roofit} & \roofit \\
\texttt{\textbackslash root} & \root & \texttt{\textbackslash spice} & \spice & \texttt{\textbackslash urania} & \urania \\
\end{tabular*}

\subsubsection{Languages}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash cpp} & \cpp & \texttt{\textbackslash ruby} & \ruby & \texttt{\textbackslash fortran} & \fortran \\
\texttt{\textbackslash svn} & \svn & \texttt{\textbackslash git} & \git & \texttt{\textbackslash latex} & \latex \\
\end{tabular*}

\subsubsection{Data processing}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash kbit} & \kbit & \texttt{\textbackslash kbps} & \kbps & \texttt{\textbackslash kbytes} & \kbytes \\
\texttt{\textbackslash kbyps} & \kbyps & \texttt{\textbackslash mbit} & \mbit & \texttt{\textbackslash mbps} & \mbps \\
\texttt{\textbackslash mbytes} & \mbytes & \texttt{\textbackslash mbyps} & \mbyps & \texttt{\textbackslash gbit} & \gbit \\
\texttt{\textbackslash gbps} & \gbps & \texttt{\textbackslash gbytes} & \gbytes & \texttt{\textbackslash gbyps} & \gbyps \\
\texttt{\textbackslash tbit} & \tbit & \texttt{\textbackslash tbps} & \tbps & \texttt{\textbackslash tbytes} & \tbytes \\
\texttt{\textbackslash tbyps} & \tbyps & \texttt{\textbackslash dst} & \dst &  \\
\end{tabular*}

\subsection{Detector related}
\subsubsection{Detector technologies}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash nonn} & \nonn & \texttt{\textbackslash ponn} & \ponn & \texttt{\textbackslash nonp} & \nonp \\
\texttt{\textbackslash cvd} & \cvd & \texttt{\textbackslash mwpc} & \mwpc & \texttt{\textbackslash gem} & \gem \\
\end{tabular*}

\subsubsection{Detector components, electronics}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tell1} & \tell1 & \texttt{\textbackslash ukl1} & \ukl1 & \texttt{\textbackslash beetle} & \beetle \\
\texttt{\textbackslash otis} & \otis & \texttt{\textbackslash croc} & \croc & \texttt{\textbackslash carioca} & \carioca \\
\texttt{\textbackslash dialog} & \dialog & \texttt{\textbackslash sync} & \sync & \texttt{\textbackslash cardiac} & \cardiac \\
\texttt{\textbackslash gol} & \gol & \texttt{\textbackslash vcsel} & \vcsel & \texttt{\textbackslash ttc} & \ttc \\
\texttt{\textbackslash ttcrx} & \ttcrx & \texttt{\textbackslash hpd} & \hpd & \texttt{\textbackslash pmt} & \pmt \\
\texttt{\textbackslash specs} & \specs & \texttt{\textbackslash elmb} & \elmb & \texttt{\textbackslash fpga} & \fpga \\
\texttt{\textbackslash plc} & \plc & \texttt{\textbackslash rasnik} & \rasnik & \texttt{\textbackslash elmb} & \elmb \\
\texttt{\textbackslash can} & \can & \texttt{\textbackslash lvds} & \lvds & \texttt{\textbackslash ntc} & \ntc \\
\texttt{\textbackslash adc} & \adc & \texttt{\textbackslash led} & \led & \texttt{\textbackslash ccd} & \ccd \\
\texttt{\textbackslash hv} & \hv & \texttt{\textbackslash lv} & \lv & \texttt{\textbackslash pvss} & \pvss \\
\texttt{\textbackslash cmos} & \cmos & \texttt{\textbackslash fifo} & \fifo & \texttt{\textbackslash ccpc} & \ccpc \\
\end{tabular*}

\subsubsection{Chemical symbols}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash cfourften} & \cfourften & \texttt{\textbackslash cffour} & \cffour & \texttt{\textbackslash cotwo} & \cotwo \\
\texttt{\textbackslash csixffouteen} & \csixffouteen & \texttt{\textbackslash mgftwo} & \mgftwo & \texttt{\textbackslash siotwo} & \siotwo \\
\end{tabular*}

\subsection{Special Text }
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash eg} & \eg & \texttt{\textbackslash ie} & \ie & \texttt{\textbackslash etal} & \etal \\
\texttt{\textbackslash etc} & \etc & \texttt{\textbackslash cf} & \cf & \texttt{\textbackslash ffp} & \ffp \\
\texttt{\textbackslash vs} & \vs &  \\
\end{tabular*}



==> principles.tex <==
\section{General principles}

The main goal is for a paper to be clear. It should be as brief as
possible, without sacrificing clarity. For all public documents,
special consideration should be given to the fact that the reader will
be less familiar with \lhcb than the author.

Here follow a list of general principles that should be adhered to:
\begin{enumerate}

\item Choices that are made concerning layout and typography
  should be consistently applied throughout the document.

\item Standard English should be used (British rather than American)
  for LHCb notes and preprints. Examples: colour, flavour, centre,
  metre, modelled and aluminium. Words ending on -ise or -isation
  (polarise, hadronisation) can be written with -ize or -ization ending but should be consistent.
  The punctuation normally follows the closing quote mark of quoted text, 
  rather than being included before the closing quote.
  Footnotes come after punctuation. 
  Papers to be submitted to an American journal can be written in American
  English instead. Under no circumstance should the two be mixed.

\item Use of jargon should be avoided where possible. ``Systematics'' are ``systematic
  uncertainties'', ``L0'' is ``hardware trigger'', Monte-Carlo'' is ``simulation'', ``penguin'' diagrams
  are best introduced with an expression like ``electroweak loop (penguin) diagrams'', ``cuts'' are ``selection requirements''. The word ``error'' is ambiguous as it can mean the difference between the true and measured values or your estimate thereof. The same applies to event, that we usually take to mean the whole $pp$ collision; candidate or decay can be used instead.''

\item It would be good to avoid using quantities that are internal jargon and/or 
  are impossible to reproduce without the full simulation, \ie\ instead of ``It is 
  required that $\chisqvtx<3$'', to say ``A good quality vertex is required''; 
  instead of ``It is required that $\chisqip>16$'', to say ``The track is 
  inconsistent with originating from a PV''; instead of ``A DLL greater 
  than 20 is required'' say to ``Tracks are required to be identified as kaons''.
  However, experience shows that some journal referees ask for exactly this 
  kind of information, and to safeguard against this, one may consider given 
  some of it in the paper, since even if the exact meaning may be LHCb-specific, 
  it still conveys some qualitative feeling for the significance levels required 
  in the varies steps of the analysis.   
 
\item \latex should be used for typesetting. Line numbering should be
  switched on for drafts that are circulated for comments.

\item The abstract should be concise, and not include citations or
  numbered equations, and should give the key results from the paper.

\item Apart from descriptions of the detector, the trigger and the
  simulation, the text should not be cut-and-pasted from other sources
  that have previously been published.

\item References should usually be made only to publicly accessible
  documents. References to LHCb conference reports and public notes
  should be avoided in journal publications, instead including the
  relevant material in the paper itself.

\item The use of tenses should be consistent. It is recommended to
  mainly stay in the present tense, for the abstract, the description
  of the analysis, \etc; the past tense is then used where necessary,
  for example when describing the data taking conditions.

\item It is recommended to use the passive rather than active voice:
  ``the mass is measured'', rather than ``we measure the mass''.
  Limited use of the active voice is acceptable, in situations where
  re-writing in the passive form would be cumbersome, such as for the
  acknowledgements.  Some leeway is permitted to accommodate different
  author's styles, but ``we'' should not appear excessively in the
  abstract or the first lines of introduction or conclusion.

\item A sentence should not start with a variable, a particle or an acronym.
 A title or caption should not start with an article. 

\item Incorrect punctuation around conjunctive adverbs and the use of 
dangling modifiers are the two most common mistakes of English grammar
in LHCb draft papers. If in doubt, read the wikipedia articles on 
conjunctive adverb and dangling modifier.  

\item When using natural units, at the first occurrence of an energy unit
      that refers to momentum or a radius, add a footnote: ``Natural units
      with $\hbar=c=1$ are used throughout.'' Do this even when somewhere
      a length is reported in units of mm. It's not 100\% consistent, but
      most likely nobody will notice. The problem can be trivially avoided
      when no lengths scales in natural units occur, by omitting the 
      $\hbar$ from the footnote text.

\item Papers dealing with amplitude analyses and/or resonance parameters, 
      other than masses and lifetimes, should use natural units,
      since in these kind of measurements widths are traditionally 
      expressed in MeV and radii in GeV$^{-1}$. It's also the convention
      used by the PDG. 

\item Papers quoting upper limits should give the both the 90\% and
  95\% confidence level values in the text. Only one of these needs to
  be quoted in the abstract and summary.
\end{enumerate}


==> supplementary_templ.tex <==
\section{Inclusion of supplementary material}
\label{sec:Supplementary}

Three types of supplementary material should be distinguished:
\begin{itemize}
\item{A regular appendix: lengthy equations or long tables are sometimes
better put in an appendix in order not to interrupt the main flow of a paper.
Appendices will appear in the final paper, on arXiv
and on the CDS record and should be considered integral
part of a paper, and are thus to be reviewed like the rest of the paper.
An example of an LHCb paper with an appendix is Ref.~\cite{LHCb-PAPER-2013-070}.
}
\item{Supplementary material for CDS: plots or tables that 
would make the paper exceed the page limit or are
not appropriate to include in the paper itself,
but are desirable to be shown in public
should be added to the paper drafts in an appendix, and
removed from the paper before submitting to arXiv or the journal.
See Appendix~\ref{sec:Supplementary-App} for further instructions.
Examples are: comparison plots of the new result with older results,
plots that illustrate cross-checks.
An example of an LHCb paper with supplementary material for CDS 
is Ref.~\cite{LHCb-PAPER-2013-035}.
Supplementary material for CDS cannot be referenced in the paper.
Supplementary material should be included in the draft paper to be
reviewed by the collaboration.
}
\item{Supplementary material for the paper. This is usually called ``supplemental material'', which distinguishes it from supplementary material for CDS only. Most journals allow
to submit files along with the paper that will not be part of the
text of the article, but will be stored on the journal server.
Examples are plain text files with numerical data corresponding to the plots
in the paper. 
The supplemental material should be cited in the paper by including a reference
which should say ``See supplemental material at [link] for [give brief description of material].''
The journal will insert a specific link for [link]. The arXiv version will usually include the supplemental material as part of the paper and so should not contain the words ``at [link]''.
Supplemental material should be included in the draft paper to be
reviewed by the collaboration.
An example of an LHCb paper with supplemental material 
is Ref.~\cite{LHCb-PAPER-2015-029}
}
\end{itemize}



==> title-LHCb-ANA.tex <==
% $Id: title-LHCb-ANA.tex 39841 2013-07-26 10:31:08Z roldeman $
% ===============================================================================
% Purpose: LHCb-ANA Note title page template
% Author: 
% Created on: 2010-10-05
% ===============================================================================

%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  TITLE PAGE  %%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{titlepage}

% Header ---------------------------------------------------
\vspace*{-1.5cm}

\noindent
\begin{tabular*}{\linewidth}{lc@{\extracolsep{\fill}}r@{\extracolsep{0pt}}}
\ifthenelse{\boolean{pdflatex}}% Logo format choice
{\vspace*{-1.2cm}\mbox{\!\!\!\includegraphics[width=.14\textwidth]{figs/lhcb-logo.pdf}} & &}%
{\vspace*{-1.2cm}\mbox{\!\!\!\includegraphics[width=.12\textwidth]{figs/lhcb-logo.eps}} & &}
 \\
 & & LHCb-ANA-20XX-YYY \\  % ID 
 & & \today \\ % Date - Can also hardwire e.g.: 23 March 2010
 & & \\
\hline
\end{tabular*}

\vspace*{4.0cm}

% Title --------------------------------------------------
{\normalfont\bfseries\boldmath\huge
\begin{center}
% DO NOT EDIT HERE. Instead edit macro in main.tex to keep metadata correct
  \papertitle
\end{center}
}

\vspace*{2.0cm}

% Authors -------------------------------------------------
\begin{center}
% If changing to list here, make pdfauthors in main.tex a comma
% separated list with the same names. Otherwise metadata in file will be wrong.
\paperauthors$^1$.
\bigskip\\
{\normalfont\itshape\footnotesize
$ ^1$Imperial College London, London, United Kingdom\\
}
\end{center}

\vspace{\fill}

% Abstract -----------------------------------------------
\begin{abstract}
  \noindent
  Guidelines for the preparation of LHCb documents are given. This is
  a ``living'' document, that should reflect our current practice. It
  is expected that these guidelines are implemented for papers already
  before they go into the first collaboration wide review. Please
  contact the Editorial Board chair if you have suggestions for
  modifications.
\end{abstract}

\vspace*{2.0cm}
\vspace{\fill}

\end{titlepage}


\pagestyle{empty}  % no page number for the title 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  EOD OF TITLE PAGE  %%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%  empty page follows the title page ----
\newpage
\setcounter{page}{2}
\mbox{~}

\cleardoublepage

